Efficient Recovery of Sparse Graph Signals from Graph Filter Outputs

This paper investigates the recovery of a node-domain sparse graph signal from the output of a graph filter. This problem, which is often referred to as the identification of the source of a diffused sparse graph signal, is seminal in the field of graph signal processing (GSP). Sparse graph signals can be used in the modeling of a variety of real-world applications in networks, such as social, biological, and power systems, and enable various GSP tasks, such as graph signal reconstruction, blind deconvolution, and sampling. In this paper, we assume double sparsity of both the graph signal and the graph topology, as well as a low-order graph filter. We propose three algorithms to reconstruct the support set of the input sparse graph signal from the graph filter output samples, leveraging these assumptions and the generalized information criterion (GIC). First, we describe the graph multiple GIC (GM-GIC) method, which is based on partitioning the dictionary elements (graph filter matrix columns) that capture information on the signal into smaller subsets. Then, the local GICs are computed for each subset and aggregated to make a global decision. Second, inspired by the well-known branch and bound (BNB) approach, we develop the graph-based branch and bound GIC (graph-BNB-GIC), and incorporate a new tractable heuristic bound tailored to the graph and graph filter characteristics. In addition, we propose the graph-based first order correction (GFOC) method, which improves existing sparse recovery methods by iteratively examining potential improvements to the GIC cost function by replacing elements from the estimated support set with elements from their one-hop neighborhood. In addition, we investigate the application of our graph-based sparse recovery methods in blind deconvolution scenarios where the graph filter is unknown.

==> b_sections/a_title.tex <==
\title{Recovery of Sparse Graph Signals from Graph Filter Outputs}
%authors
\author{Gal Morgenstern~\IEEEmembership{Student Member,~IEEE},
	and~Tirza~Routtenberg,~\IEEEmembership{Senior Member,~IEEE}  % <-this % stops a space
%thanks
\thanks{G. Morgenstern and T. Routtenberg are with the School of ECE, Ben-Gurion University of the Negev, Beer Sheva, Israel (e-mail: \{galmo@post.;tirzar\}@bgu.ac.il). T. Routtenberg is also with the ECE Department at Princeton University, Princeton, NJ. This work is partially supported by the Israel Science Foundation (grant No. 1148/22), the Jabotinsky Scholarship from the Israel Ministry of Technology and Science, and the Israel Ministry of National Infrastructure and Energy}}
% The paper headers
\markboth{Journal of \LaTeX\ Class Files,~Vol.~14, No.~8, August~2015}%
{Shell \MakeLowercase{\textit{et al.}}: Bare Advanced Demo of IEEEtran.cls for IEEE Computer Society Journals}



% make the title area
\maketitle

%\IEEEtitleabstractindextext{
\begin{abstract}
In this study, we investigate sparse recovery in graphical settings where signal values are distributed over the vertices of an undirected graph. 
We aim to recover a sparse signal from the noisy excitations of a graph filter, which is used to model a graphical process performed on the signal.
We approach this problem by casting it as a hypothesis-testing problem and then applying the well-known generalized information criterion (GIC). 
Since a direct solution for the GIC problem requires an exhaustive search, we propose two low-complexity methods.
These methods leverage the double sparsity imposed by the graph signal and the underlying graph
and provide a trade-off between support estimation performance and computational complexity. 
To further improve the support recovery results, we have created a low-complexity correction algorithm that takes an estimated support as input and checks whether a better solution is available in the estimated support local neighborhood over the graph.
The correction method can also be applied to standard sparse approximation methods. 
We have also provided a theoretical analysis of the sparse recovery problem in graphical settings where the graph filter is selected to be the graph Laplacian matrix. Finally, we evaluated the performance of our methods against the orthogonal matching pursuit and the Lasso algorithms, and our methods were superior.
\end{abstract}

% Note that keywords are not normally used for peer-reviewed papers.
\begin{IEEEkeywords}
Sparse signal estimation, support recovery, double sparsity, generalize information criterion, graph signals, graph filters
\end{IEEEkeywords}%}


==> b_sections/b_introduction.tex <==

\section{Introduction}
\label{sec:introduction}

The field of \ac{gsp} has attracted significant attention in recent years due to the growing importance of networked data in various domains,
such as brain imaging \cite{huang2016graph} and sensor networks \cite{olfati2005consensus}.
\ac{gsp} expands upon \ac{dsp} principles, enabling data processing associated with arbitrary graphs \cite{ortega2018graph,shuman2013emerging,sandryhaila2013discrete}, with concepts such as sampling and recovery of graph signal \cite{tanaka2020sampling,marques2015sampling,chen2015signal,sagi2022gsp,kroizer2022bayesian,amar2023widely}, graph Fourier transform (GFT), graph smoothness \cite{dabush2023verifying}, and graph filter design \cite{shuman2013emerging,isufi2016autoregressive}. 
However, insufficient attention has been given to addressing solutions for sparse recovery problems in graphical settings.

Sparse recovery techniques have been a major area of research for the past two decades (see, for example, \cite{Chen_Donoho_2001,Tropp_2004,elad2010sparse,donoho2005stable} and references therein). These techniques can be classified into three main categories \cite{marques2018review}: convex relaxations \cite{Chen_Donoho_2001,tibshirani1996regression,efron2004least,candes2007dantzig, donoho2009message}, non-convex optimization techniques \cite{wipf2004sparse,gorodnitsky1997sparse, chartrand2008iteratively}, and greedy algorithms \cite{mallat1993matching,Tropp_2004,cai2011orthogonal, dai2009subspace, blumensath2008gradient }.
Among the widely used approaches is the Lasso method \cite{tibshirani1996regression} and Orthogonal Matching Pursuit (OMP) \cite{cai2011orthogonal}. Researchers have also proposed specialized solutions for scenarios where prior information is available about either the signal's sparsity pattern or the dictionary matrix's structure. For instance, some studies consider the dictionary matrix itself to be sparse \cite{berinde2008sparse,gilbert2010sparse}, while others focus on reconstructing a sparse signal from Fourier measurements \cite{eldar2014sparse,jaganathan2012recovery,hassanieh2012nearly}. Block sparse signals, characterized by clusters of non-zero entries, were introduced in \cite{eldar2010block}. In \cite{plumbley2009sparse}, sparse representations are advocated for audio signals.
In \cite{morgenstern2020structuralconstrained}, sparsity patterns are discussed in the context of power system cyber-security. 
In contrast to these tailored solutions, specified solutions that consider the underlying graphical structure are not always available in a variety of \ac{gsp} applications that include sparse graph signals. 

Sparsity patterns arise in a variety of graphical settings \cite{haupt2008compressed}. 
In the area of network tomography sparse signals are used to represent the properties of the graph edges \cite{xu2011compressive,cheraghchi2012graph}.
In social networks, identifying the $k$-top influential vertices, 
has been formulated as a sparse recovery problem \cite{kourtellis2013identifying}. 
Diffusion processes that originate from a sparse set of vertices are used to model a variety of
problems such as finding the source of a disease \cite{newman2002spread, pinto2012locating}, 
anomaly detection \cite{schizas2009distributed}, opinion forming \cite{rainer2002opinion, patterson2010interaction},
brain connectivity analysis \cite{kramer2008emergent}, and cybersecurity in power systems \cite{morgenstern2023protection,drayer2019detection}.
Locating the source of a diffusion process has been addressed in \cite{shah2011rumors, shah2010detecting}
for Bayesian frameworks.
In \cite{segarra2016blind, ramirez2021graph, shuman2018distributed, tenorio2023blind}, this problem
has been generalized to \ac{gsp} applications, 
such as blind deconvolution and sampling. 
Specifically, the problem was restated as the recovery of a sparse graph signal
from the output of a graph filter. 
However, in most existing methods that can be restated in this form, sparsity is typically considered either in the signal or the graph, but not in both aspects simultaneously. As a consequence, these approaches may not fully exploit the potential benefits of the sparse and graphical structures inherent in the data.

In this paper, we investigate the problem of recovering sparse signals over sparse graphs.
We aim to recover the signal from the excitations of a linear graph filter. To achieve this, we cast the sparse recovery problem as a hypothesis-testing problem and introduce the well-known \ac{gic} criterion.
We propose two new sparse recovery methods: 1) the \ac{gmgic; and 2) the \ac{gbgic} methods. 
Both methods utilize the double sparsity imposed by the graph and graph signal. 
The \ac{gmgic} method, which we first introduced in [\color{red}ref\color{black}]\footnote{This conference article is yet to be published. In the meantime, should I upload the conference on Arxiv?}, identifies and partitions a set of vertices suspected to contain the sparse graph signal support and then applies a local \ac{gic} on each partition.
To clarify, the \ac{gic} criterion is resolved by performing an exhaustive search within each partition.
Meanwhile, the \ac{gbgic} is an iterative algorithm based on binary search trees. 
We also introduce the \ac{gfoc} method. 
The \ac{gfoc} is a low-complexity correction algorithm that takes an estimated support of the graph signal as input and examines whether a better solution exists in the estimated support's local neighborhood over the graph.
Additionally, we conduct a theoretical analysis of the sparse recovery problem, considering the graph Laplacian matrix as the graph filter.
Finally, we provide a performance evaluation of the proposed methods. 
The results show that the \ac{gmgic} and{\ac{gbgic} methods can achieve support recovery comparable to the \ac{gic} benchmark,whicht requires an exhaustive search on all the possible supports, while also outperforming the Lasso and \ac{omp} methods. 
Moreover, these methods have the advantage of being low-complexity compared to directly solving the \ac{gic} criterion. Additionally, simulations demonstrate that the \ac{gfoc} can effectively enhance the estimation results of the support recovery methods with minimal added complexity burden.

The paper is organized as follows. Section \ref{sec; problem} presents the necessary background and underlines the problem formulation. The proposed techniques for support recovery of sparse graph signals are presented in Section \ref{Sec; theory sparse recovery}. In Section \ref{sec; theoretical; analysis}, we analyze the sparse recovery problem for the case that the graph filter is selected to be a graph Laplacian matrix. Finally, we evaluate the performance in Section \ref{sec; simulations} and conclude our findings in Section \ref{sec; conclusions}.


{\em{Notations:}} 
In the rest of this paper, vectors and matrices are denoted by boldface lowercase and uppercase letters.
%The identity matrix is denoted by $\Imat$. 
The $(\none,\ntwo)$th element of the matrix $\filter$ is denoted by $H_{\none,\ntwo}$. 
The vector ${\signal}_{\signalsupport}$ is a subvector of $\signal$ with the elements indexed by the set $\signalsupport$, 
and $\Fmat_{\signalsupport}$ is the submatrix of $\Fmat$ consisting of the {\em{columns}} indexed by $\signalsupport$. 
The projection matrix over the subspace $\text{col}(\Fmat_{\signalsupport})$
is given by $\proj{\signalsupport}=\filter_{\signalsupport}(\filter_{\signalsupport}^T\filter_{\signalsupport})^{-1}\filter_{\signalsupport}^T$. 
%The cardinality of the set $\signalsupport$ is denoted by $\lvert\signalsupport \rvert$. 
The operators $\norm{\cdot}$, $\norm{\cdot}_1$, $\norm{\cdot}_0$, and $\card{\cdot}$ denote the Euclidean norm, 
$\ell_1$ norm, zero seminorm, and set cardinality. 





==> b_sections/c_background_graph.tex <==
\subsection{Background: Graph and Graph Filters } \label{sec; graph}
%Graph and graph filter properties are crucial in our analysis. 
Consider an undirected weighted graph  $\graph$ , consisting of a set of vertices $\nodes$, a set of edges $\edges$, 
and a set of weights $\{\edgeweight_{e}\}_{e\in\edges}$. 
A signal over the graph is a mapping between the graph vertices to an $\card{\nodes}\times 1$ real vector, i.e. 
\be \label{eq; graph signal}
\signal: \nodes\rightarrow \mathbb{R}^{\card{\nodes}}.
\ee
This signal can be shifted using a \ac{gso}, $\dimsquare{\gso}{\card{\nodes}}$, which provides a new graph signal, $\gso\signal$, addressed as the shifted signal. 
The \ac{gso} matrix, which is based on the graph structure and the graph edge weights, satisfies 
\be\label{eq; gso}
  \gsoentry_{\none,\ntwo}=0, ~ ~~\text{if}~\geo{\none}{\ntwo}>1,~~~\forall \none,\ntwo\in\nodes,
\ee
where $\geo{\none}{\ntwo}$ is the geodesic distance between vertices $\none$ and $\ntwo$ over the graph $\graph$.
The geodesic distance between two vertices refers to the number of edges on the minimal path that connects these vertices. 
According to the condition in \eqref{eq; gso},
the nonzero values of $\entrymat{\gso}{\none}{\ntwo}$ are located in the entries that satisfy $\none=\ntwo$ or $\edge{\none}{\ntwo}\in\edges$. 
Consequently, each element of the shifted signal is a linear combination of the signal elements in its local neighborhood:
\be \label{eq; gso linear}
[\gso\signal]_{\none}= \sum_{\ntwo\in\firstnei{\none}} \gsoentry_{\none,\ntwo} \signalentry_{\ntwo},  
\ee
where $\firstnei{\none}=\{\ntwo\in\nodes:~0\le\geo{\none}{\ntwo}\le 1\}$. 
More generally, a signal may be filtered by applying a graph filter, $\dimsquare{\filter}{\card{\nodes}}$, providing a new graph signal, $\filter\signal$, addressed as the filtered signal. 
We consider invariant graph filters that are defined as  
polynomials of the \ac{gso},\cite{shuman2013emerging,sandryhaila2013discrete}:
\be \label{eq; graph filter}
\filter=h_0\Imat+h_1\gso+\ldots +h_{\filterdeg}\gso^{\filterdeg},
\ee
where $h_0,\ldots,h_{\filterdeg}$ are the coefficients of the graph filter and $1\leq  \filterdeg\leq \card{\nodes} $  is the graph filter order. 
By substituting \eqref{eq; gso} in \eqref{eq; graph filter} it can be verified that 
\be \label{eq; F prop}
\filterentry_{\none,\ntwo}=\sum_{i=0}^\Psi h_i [\gso^i]_{k,m}=0,~~~\text{if}~\geo{\none}{\ntwo}>\filterdeg,~~~\forall \none,\ntwo\in\nodes.
\ee
Consequently, we obtain that each element of the filtered signal is a linear 
combination of the signal elements in its closed $\Psi$-local neighborhood:
\be \label{eq; graph filter linear}
[\filter\signal]_{\none}= \sum_{\ntwo\in\nei{\Psi}{\none}} \filterentry_{\none,\ntwo} \signalentry_{\ntwo}, 
\ee
where 
\be  \label{eq; local neighberhood}
\nei{\filterdeg}{\none}=\{\ntwo\in\nodes:~0\le \geo{\none}{\ntwo}\le \filterdeg\} 
\ee
includes all the vertices in the closed $\filterdeg$-local neighborhood of vertex $\none$. 



==> b_sections/c_background_sparse.tex <==


\section{Problem Formulation} \label{sec; problem}

In Subsection \ref{sec; sparse recovery}, we demonstrate that sparse recovery can be framed as a support recovery problem, and its solution can be achieved using the \ac{gic} criterion. In Subsection \ref{sec; graph}, we provide relevant background on graph signals and graph filters. 
%While these two subsections do not make explicit references to each other, they both contribute to the problem formulation in Section \ref{sec; problem}.


\subsection{Background: Recovery of Sparse Signals} \label{sec; sparse recovery}
We are interested in recovering the signal, $\signal$, from the following set of measurements
\be \label{eq; model}
\measurements=\dictionary\signals+\noise,
\ee
where $\dictionary$ is denoted as the sparse dictionary matrix. 
The vector $\dimvec{\noise}{\card{\nodes}}$
with covariance matrix $\noisecov$, i.e. $\noise\sim\normal{\zerovec}{\noisecov}$.
In addition, the signal is assumed to be sparse
and this restriction is formulated by 
\be \label{eq; sparsity restriction}
\norm{\signals}_0\leq \sparsityterm,
\ee
where $\norm{\cdot}_0$ is the $\ell_0$ semi-norm and $\sparsityterm$ indicates the sparsity level.
Hence, there exists a set of vertices, addressed as the signal support set and denoted by $\signalsupport_t$, such that 
\be \label{eq; support set}
\entryvec{\signals}{\none}=0,~\none \in \{\nodes\setminus\signalsupport_t\}.
\ee
Therefore, based on \eqref{eq; model} and \eqref{eq; support set}, we formulate the recovery problem 
as (Eq. (1) in \cite{Tropp_2004}):
\be \label{eq; SR 2}
(\hat{\signals},\hat{\signalsupport})=\underset{\card{\signalsupport} \le \sparsityterm}{\min}
\underset{~\dimvec{\signals_{\signalsupport}}{\card{\signalsupport}}}{\min} ~\norm{ \measurements-
\dictionary_\signalsupport \signals_{\signalsupport}} ^2.%~s.t.~ \signals_{\signalsupport^c}=\zerovec.
\ee
By substituting the weighted least squares solution (see equation 8.10 on page 225 in \cite{kay1993fundamentals}),
\be \label{eq; WLS}
\hat{\signals}_{\signalsupport}=\arg\underset{\dimvec{\signals_{\signalsupport}}{\card{\signalsupport}}}{\min} ~\norm{ \measurements-
\dictionary_\signalsupport \signals_{\signalsupport}}
^2=(\dictionary_{\signalsupport}^T\dictionary_{\signalsupport})^{-1}\dictionary^T_{\signalsupport}\measurements,
\ee
in \eqref{eq; SR 2},
we obtain the support recovery problem
\be \label{eq; sup}
\begin{aligned}
\hat{\signalsupport}&=\underset{\card{\signalsupport} \le \sparsityterm}{\min}\norm{ \measurements-\projs{\signalsupport}\measurements}^2 =\underset{\card{\signalsupport} \le \sparsityterm}{\max}\norm{\projs{\signalsupport}\measurements}^2,
\end{aligned}
\ee
where $\projs{\signalsupport}=\projection{\dictionary_{\signalsupport}}$ is the projection matrix onto the subspace $\text{col}(\dictionary_{\signalsupport})$.
The last equality in \eqref{eq; sup} is obtained by using the projection matrix property $\norm{\measurements-\projs{\signalsupport}\measurements}^2= \norm{\measurements}^2-\norm{\projs{\signalsupport}\measurements}^2$ (see Theorem 2.22 on page 46 in \cite{yanai2011projection}), removing the constant $\norm{\measurements}^2$, and rearranging the optimization problem. 

The support recovery problem in \eqref{eq; sup} can be viewed as a 
multiple hypothesis testing
%model selection 
problem, 
where in each hypothesis the sparse signal is assigned with a different support set from $\{\signalsupport\in\mathcal{V}:~\lvert \signalsupport\rvert\le s\}$.
Therefore, we use the well-known \ac{gic} model selection method,
%in noisy settings. 
 which is a generalization of various criteria, such as the \ac{aic}
 and the \ac{mdl}, and is given by\cite{stoica2004model}
\be \label{eq; gic}
\hat{\signalsupport}=\underset{\card{\signalsupport} \le \sparsityterm}{\max}\norm{\projs{\signalsupport}\measurements}^2-\penaltygic{\signalsupport}.
\ee
Compared to \eqref{eq; sup}, the \ac{gic} in \eqref{eq; gic} includes an additional component, $\penaltygic{\signalsupport}$, which is a penalty function that depends on the support cardinality. 
This penalty term mitigates the risk of over-fitting.
After solving \eqref{eq; gic},
the sparse signal recovery solution can be obtained by substituting $\hat{\signalsupport}$ in \eqref{eq; WLS}.
However, 
in practice, solving \eqref{eq; gic} 
is infeasible due to the exponential increase in the number of candidate supports
\ac{wrt} the network size. 


%$\forall k,m\in\mathcal{V}$,

==> b_sections/c_problem_formulation.tex <==



\subsection{Problem Formulation: Recovery of Sparse Graph Signals} \label{sec; sparse graph signals}
We consider the support recovery problem in \eqref{eq; gic}, which is based on the measurement model in \eqref{eq; model},
for the case that the dictionary matrix is the graph filter defined in \eqref{eq; graph filter}, hence $\dictionary=\filter$, 
and the sparse signal is the graph signal defined in \eqref{eq; graph signal}, hence $\signals=\signal$. 
In addition, we consider the following assumptions on the graphical setting: 
\begin{enumerate}[label=\textbf{A.\arabic*}, leftmargin=1cm,topsep=2.5pt]
\item \label{A; graph sparse} The graph is sparse; i.e., the number of graph edges, $\lvert  \edges \rvert$, is in the order of  $O(\lvert \mathcal{V}\rvert)$.
%is in the  order of number of vertices, $\lvert \edges \rvert=O(\lvert \mathcal{V}\rvert)$.
\item \label{A; graph connectivity} The average geodesic distance over the graph, 
 \[\frac{1}{2\card{\nodes}(\card{\nodes}-1)}\sum_{\none,\ntwo\in\nodes} \geo{\none}{\ntwo},\]
is relatively large. 
\item \label{A; filter degree} The graph filter degree $\filterdeg$ is small \ac{wrt} the system size, i.e., 
$ \filterdeg\ll\card{\nodes} $.
\item  \label{A; filter coefficients} The coefficients of the graph filter, $h_i$, $i=0,\ldots $, decay by $\abs{ h_i}=\rate\abs{h_{i+1}}$, where $0<\rate<1$ is a user-defined parameter controlling the rate of decay.  
\end{enumerate}
%Assumptions \ref{A; graph sparse}-\ref{A; graph connectivity} refer to the underlying graph while Assumptions \ref{A; filter degree}-\ref{A; filter coefficients}
%refer to the graph filter. 
According to Assumptions \ref{A; graph sparse}-\ref{A; graph connectivity}, the connectivity pattern of the underlying graph is expected to exhibit a local behavior where only vertices that are geographically close to each other are likely to be connected by an edge.
For example, graphs of infrastructure networks, such as power systems and transportation systems, often satisfy
this behavior.
When we combine Assumptions \ref{A; graph sparse}-\ref{A; graph connectivity} with Assumption \ref{A; filter degree}, it implies that the closed $\Psi$-local neighborhood of a vertex, defined in \eqref{eq; local neighberhood}, consists of only a small portion from the graph vertices. 
Additionally, the combination of the result in \eqref{eq; graph filter linear} with Assumptions \ref{A; graph sparse}-\ref{A; filter coefficients} means that the values of the filtered signal can be related to the location of their indices over the graph. Specifically, this implies that, in general, the values will be larger for the filtered signal entries with indices closer to the vertices in $\signalsupport_t$.

%From the above assumptions and the sparsity constraint in \eqref{eq; support set} we draw the following two conclusions. 
%First, the set of vertices in which the filtered signal, $\filter\signal$, holds significant information on the signal, $\xvec$, 
%includes only a small portion of the vertices over the graph. 
%Second, if the signal support, $\signalsupport_t$, can be separated to subsets distant one from the other over the graph, there mutual influence is expected to be %small.

%Hence, it could be assumed that the information required to evaluate the different subsets are located in different indices of the filtered signal, $\Hmat\xvec$. 


==> b_sections/d_analysis.tex <==
\subsection{Analysis} \label{sec; sparse; analysis}

As a direct consequence of \eqref{eq; F prop}, we can deduce that if the geodesic distance between vertices $\none$ and $\ntwo$ is larger than $2\filterdeg$, i.e. $\geo{\none}{\ntwo}>2\filterdeg$, then the two graph filter columns corresponding to these vertices, i.e. $\filter_{\none}$ and $\filter_{\ntwo}$, are orthogonal.
Hence, we obtain that  
\be \label{eq; F prop 2}
\filter_{\ntwo}^T\filter_{\none}=  \sum_{\iterone\in\nodes} \filterentry_{\ntwo, \iterone}\filterentry_{\none,\ntwo}
= 0,
\ee
  $\forall \none,\ntwo\in\nodes$ such that $\geo{\none}{\ntwo}>2\filterdeg$.
% In this context, $\filter_{\ntwo}$ is the $m$th column of $\filter$.
That is because
 $\geo{\none}{\ntwo}>2\filterdeg$, then $\geo{\ntwo}{\iterone}>\filterdeg$
and/or $\geo{\none}{\iterone}>\filterdeg$, $\forall \iterone\in\nodes$.
Thus, for any element in the summation $\filterentry_{\ntwo, \iterone}=0$ and/or $\filterentry_{\none,\iterone}=0$.

\subsubsection{Rating Dictionary Atoms}

Based on \eqref{eq; F prop 2} we provide the following theorem:
\begin{thm}\label{thm; projection}
Suppose the graph signal $\signal$ only takes non-zero values over the support $\signalsupport_t$. Then, the projection of the filtered signal, $\filter\signal$, onto the single-vertex measurement subspace $\text{col}(\filter_{\ntwo})$ satisfies
\be \label{eq; filtered 0}
\proj{\ntwo}\filter\signal=\proj{\ntwo}\filter_{\signalsupport_t}\signal_{\signalsupport_t}=\zerovec,
\ee
$\forall \ntwo\notin \nei{2\filterdeg}{\signalsupport_t}$, 
where 
\be \label{eq; neighborhood}
\begin{aligned}
\nei{2\filterdeg}{\signalsupport_t}&\define \bigcup_{\none\in\signalsupport_t} \nei{2\filterdeg}{\none} \\
&=\{\none\in\nodes:~\exists\ntwo\in\signalsupport_t:~ 0<\geo{\none}{\ntwo}\le 2\filterdeg\},
\end{aligned}
\ee
where $\nei{2\filterdeg}{\none}$ is defined in \eqref{eq; local neighberhood}.
%Hence, any vertex $\ntwo$ with a geodesic distance larger than $2\filterdeg$ then any of the vertices in $\signalsupport_t$
%satisfies \eqref{eq; filtered 0}.
The set $\nei{2\filterdeg}{\signalsupport_t}$ is referred to as the $2\filterdeg$ neighborhood of the vertex set $\signalsupport_t$. 
\end{thm}
\begin{proof}
From \eqref{eq; F prop 2}, if the geodesic distance between vertices $\none$ and $\ntwo$, $\geo{\none}{\ntwo}$, is larger than $2\filterdeg$, then we obtain
\be \label{eq; 2nd 0}
\begin{aligned}
\proj{\ntwo}\filter_{\none}
=\projection{\filter_{\ntwo}}\filter_{\none}  = \zerovec,
\end{aligned}
\ee
where $\filter_{\none}$ is the $\none$th column of $\filter$, and $\proj{\ntwo}$ is
the projection matrix onto the single-column space $\text{col}(\filter_{\ntwo})$.
 As a result, if $m\notin \nei{2\filterdeg}{\signalsupport_t}$, then left-multiplying 
 \be \label{eq; filtered signal}
\filter\signal=\filter_{\signalsupport_t}\signal_{\signalsupport_t}=\sum\limits_{\none\in\signalsupport_t} \filter_{\none}\signalentry_{\none}. 
\ee
by $\proj{\ntwo}$ results in \eqref{eq; filtered 0}.  
\end{proof}
Left-multiplying the measurement model in \eqref{eq; model} by $\proj{\ntwo}$ and substituting \eqref{eq; filtered 0} results with
\be
\label{14}
\proj{\ntwo}\measurements=\proj{\ntwo}\filter\signal+\proj{\ntwo}\noise=\proj{\ntwo}\noise
\ee
for all $\ntwo\notin \nei{2\filterdeg}{\signalsupport_t}$. 
Consequently, the dictionary atoms, i.e., graph filter columns, indexed by vertices outside the set $\nei{2\filterdeg}{\signalsupport_t}$ are not part of the sparse signal representation.
Hence, they may only represent the noise.  
Therefore, due to Assumptions \ref{A; graph sparse}-\ref{A; filter degree}, only a portion of dictionary elements can represent the sparse graph signal. These elements are the graph filter columns associated with the set $\nei{2\filterdeg}{\signalsupport_t}$.
Moreover, assuming that the graph vertices are indexed according to the ordering
\be \label{eq; ordering}
\begin{aligned}
\norm{\proj{1}\measurements}_2^2&\ge \norm{\proj{2}\measurements}_2^2\ge \ldots \\
&\ge \norm{\proj{\card{\nei{2\filterdeg}{\signalsupport_t}}}\measurements}_2^2 \ge 
 \ldots \ge \norm{\proj{\card{\nodes}}\measurements}_2^2,    
\end{aligned}
\ee
then from Assumptions \ref{A; graph sparse}, \ref{A; graph connectivity} and \ref{A; filter coefficients}  
it is expected that the vertices with lower indices are the ones closer, over the graph, to the vertices in $\signalsupport_t$. 
Furthermore, it is expected that from a certain index $\none> \card{\nei{2\filterdeg}{\signalsupport_t}}$ 
 we will obtain 
\be \label{eq; order epsilon}
\norm{\proj{\none}\measurements}_2^2\le \epsilon_1
\ee
where $\epsilon_1$ represents a relatively small value. 
Therefore, it is assumed that the representation of the sparse signal involves only a subset of dictionary atoms.
These elements are assumed to be located in the set 
\vspace{-0.1cm}\be  \label{eq; pre-screening}
\dset\define\{\ntwo\in\nodes:~\norm{ \proj{\ntwo}   \measurements} ^2  >\threshold\},
\ee
where $\threshold$ is a user-defined threshold.

\subsubsection{Observing the Signal as Multiple Sources}

Based on \eqref{eq; F prop 2} we provide the following theorem:
\begin{thm}\label{thm; partition}
Suppose that the set $\dset$ is partitioned to the subsets $\dsubsets$
such that 
\be \label{eq; partition}
\geo{\none}{\ntwo}>2\filterdeg,~\forall \none \in\dsubset{q}, ~\forall \ntwo\in\dsubset{q'},
\ee
for any two subsets $\dsubset{q}$ and $\dsubset{q'}$ from $\dsubsets$, where $q\ne q'$ and $1\leq Q \leq \sparsityterm$.
Then, the following linear decomposition is satisfied:
\be \label{eq; decomposition}
\norm{\proj{\dset}\measurements}_2^2=\sum_{q=1}^{Q} \norm{\proj{\dsubset{q}}\measurements}_2^2.
\ee
Note that if the set $\dset$ cannot be partitioned by \eqref{eq; partition} then $Q=1$ in \eqref{eq; decomposition}. 
\end{thm}
\begin{proof}
Consider any to indices $q$ and $q'$ from $\{1,2, \ldots Q\}$. 
Then, by \eqref{eq; F prop 2}, $\Hmat_{\{m\}}$ and $\Hmat_{\{k\}}$ are orthogonal 
for any selection of $\none$ from $\dsubset{q}$ and any selection of $\ntwo$ from $\dsubset{q'}$.
As a result, we obtain that the linear spaces $\text{col}(\Hmat_{\dsubset{q}})$ and $\text{col}(\filter_{\dsubset{q'}})$
are orthogonal.
Consequently, the column spaces $\{\text{col}(\filter_{\dsubset{q})}\}_{q=1}^Q$ 
 are orthogonal and the decomposition presented in \eqref{eq; decomposition} is satisfied (see Theorem $2$ on page $36$ in \cite{yanai2011projection}).)
\end{proof}
According to Theory \ref{thm; partition}, if the support of a sparse signal is situated 
such that the locations of the non-zero values of the filtered signal, $\filter\signal$, can be separated to isolated regions that maintain \eqref{eq; partition}, then the signal can be considered as a combination of multiple signals.
As a result, the support of each component in the combination can be estimated independently.
Following this note, we assume, based on Assumptions \ref{A; graph sparse}, \ref{A; graph connectivity}, and \ref{A; filter coefficients}, that if the geodesic distance between two nodes in the graph is greater than a certain scalar $\tilde{\filterdeg}$,  $\geo{\none}{\ntwo}>\tilde{\filterdeg}$,
then 
\be \label{eq; F prop smaller}
\filter_{\ntwo}^T\filter_{\none}\le \epsilon_2,
\ee
where $\epsilon_2$ represents a relatively small value.
Consequently, we assume that if the set $\dset$ is partitioned to the subsets $\dtildesubsets$
such that 
\be \label{eq; partition approx}
\geo{\none}{\ntwo}>\tilde{\filterdeg},~\forall \none\in\dtildesubset{q}, ~~~\forall \ntwo\in\dtildesubset{q'},
\ee
for any two subsets $\dtildesubset{q}$ and $\dtildesubset{q'}$  from $\dtildesubsets$, where $q\ne q'$ and $1\leq Q \leq \sparsityterm$.
Then, the following linear decomposition is approximately satisfied:
\be \label{eq; decomposition approx}
\norm{\proj{\dset}\measurements}_2^2\approx\sum_{q=1}^{Q}  \norm{\proj{\dtildesubset{q}}\measurements}_2^2.
\ee
Hence, \eqref{eq; decomposition approx} provides a relaxation to \eqref{eq; decomposition}, 
offering less restrictive conditions for the sparse signal to be treated as a combination of multiple signals,
each of which can be estimated separately.



==> b_sections/d_gbgic.tex <==
\subsection{\ac{gbgic}} \label{sec; sparse; gbgic}

In this section, we present the \ac{gbgic} method, an iterative binary tree-based search approach that utilizes equations \eqref{eq; order epsilon} and \eqref{eq; decomposition approx} to solve the support recovery problem in \eqref{eq; gic}. 
This subsection is organized as follows. 
First, we reformulate the \ac{gic} problem in Subsection \ref{sec; gbgic; prior} for the case where prior information is available on the support of the sparse graph signal. 
In Subsection \ref{sec; gbgic; bound}, we derive an upper bound for the \ac{gic} associated with the optimal solution for the problem in Subsection \ref{sec; gbgic; prior}. 
The upper bound is then used in the proposed iterative procedure presented in Subsection \ref{sec; gbgic; procedure}. 
 Additionally, we show in Subsection \ref{sec; gbgic; reduce} how to reduce the number of \ac{gic} cost function computations required for the iterative procedure. 
 Finally, we provide a discussion in \ref{sec; gbgic; discussion}.
 
\vspace{0.2cm}
\subsubsection{\ac{gic} with Prior Information } \label{sec; gbgic; prior}
We consider the case that prior information is available on the sparse graph signal, $\signal$, such that we can classify $j$ vertices, located in the range $[1,\iterone]$, based on the following rule: vertices in $\cand{\iterone}{i}\subset [1,\iterone]$ belong to the sparse signal support, $\signalsupport$, while vertices in $\{[1,\iterone]\setminus \cand{\iterone}{i}\}$ do not. We incorporate this prior information as constraints within the framework of the \ac{gic} problem presented in Equation \eqref{eq; gic}. The constrained formulation is expressed as follows:
\be \label{eq; gic with prior}
\begin{aligned}
\candsup{\iterone}{i}&=\arg\optmax{\card{\signalsupport}\le \sparsityterm} ~\gic(\signalsupport)\define\|\Pmat_{\filter_{\signalsupport}}\measurements\|^2-\rho(\card{\signalsupport})\\
&~~~~~s.t. \begin{cases}
\cand{\iterone}{i}\subseteq\signalsupport \\ 
\{[1,\iterone]\setminus\cand{\iterone}{i}\} \cap\signalsupport =\emptyset,
\end{cases}
\end{aligned}
\ee
Here, $\cand{\iterone}{i}$ represents one element in $\candset{\iterone}=\{\cand{\iterone}{1},\ldots,\cand{\iterone}{\card{\candset{\iterone}}}\}$, where $\candset{\iterone}$ represents the candidate set in iteration $j$. We will describe the candidate set $\candset{\iterone}$ further when we present the iterative procedure itself in Subsection \ref{sec; gbgic; procedure}. For $\iterone=0$, we use the convention that $[1,j]=\emptyset$ and consequently obtain that $\cand{0}{1}=\emptyset$. In this case, we return to the \ac{gic} problem in \eqref{eq; gic} with $\dictionary=\filter$.

\subsubsection{Upper Bound} \label{sec; gbgic; bound}

The optimal solution in \eqref{eq; gic with prior}, denoted by $\candsup{\iterone}{i}$, is composed of two components. 
The first component, $\cand{\iterone}{i}$, already belongs to the support $\candsup{\iterone}{i}$ and is in the range $[1,\iterone]$. 
The second component, $\{\candsup{\iterone}{i}\setminus \cand{\iterone}{i}\}$, belongs to the range $[j+1,\card{\nodes}]$ and represents a new source. 
We assume that these two components represent two different sources and approximately satisfy \eqref{eq; partition approx}. 
Therefore, when considering a linear penalty function for the \ac{gic} criterion, we can write the \ac{gic} as the superposition of $\gic$s associated with each component, 
\be
\gic(\candsup{\iterone}{i})= \gic(\cand{\iterone}{i})+\gic(\{ \candsup{\iterone}{i}\setminus \cand{\iterone}{i}\})).
\ee
We further assume that the second component, $\{\candsup{\iterone}{i}\setminus \cand{\iterone}{i}\}$, is composed of individual sources that also approximately satisfy \eqref{eq; partition approx}. 
Thus, we obtain
\be \label{eq; bounding support}
\begin{aligned}
\gic(\candsup{\iterone}{i}) &= \gic(\cand{\iterone}{i})+ \sum_{\none\in\nodes} \indicator{\{\none\in[\iterone+1,\card{\nodes}]\cap\signalsupport_{t}\}}  \gic(\none), 
% &\le \boundup{\iterone}{i},
\end{aligned}
\ee
where $\indicator{\{\cdot\}}$ is the indicator function resulting in one if the condition is maintained and zero otherwise.
We relax our assumption by replacing the equality in \eqref{eq; bounding support} with an inequality, which leads to 
\be \label{eq; bounding support inequality}
\begin{aligned}
\gic(\candsup{\iterone}{i}) &\le \gic(\cand{\iterone}{i})+ \sum_{\none\in\nodes} \indicator{\{\none\in[\iterone+1,\card{\nodes}]\cap\signalsupport_{t}\}}  \gic(\none). 
% &\le \boundup{\iterone}{i},
\end{aligned},
\ee
 Then, we bound the contribution of the individual sources by following the ordering in \eqref{eq; ordering} to obtain
 \be \label{eq; bounding up} 
\begin{aligned}
   \gic(\candsup{\iterone}{i})&\le \gic(\cand{\iterone}{i}) +(\sparsityterm-\card{\cand{\iterone}{i}})\gic(\iterone+1) \\
   &\define \boundup{\iterone}{i}.
\end{aligned}   
\ee
The upper bound $\boundup{\iterone}{i}$ represents the maximum value of $\gic(\candsup{\iterone}{i})$ for candidate $i$ in iteration $j$. 
It is the sum of the $\gic$ associated with the support $\cand{\iterone}{i}$ and the $\gic$ associated with the vertex $\iterone+1$ multiplied by $(\sparsityterm-\card{\cand{\iterone}{i}})$. 



\begin{comment}
In addition to the upper bound in \eqref{eq; bounding up} we derive a lower bound using the following claim: 
\begin{claim}
the support $\candsup{\iterone}{i}$ in \eqref{eq; gic with prior} is bounded by 
\be \label{eq; bounding low}
\gic(\candsup{\iterone}{i}) \ge \boundlow{\iterone}{i},
\ee
where 
\renewcommand{\puneq}{.}\loadeq{lowerdef}
\end{claim}
\begin{proof}
    The support set $\cand{\iterone}{i}$ is a feasible solution in \eqref{eq; gic with prior}.
    Thus, the cost function of the support that maximizes \eqref{eq; gic with prior} is greater or equal to the cost function of the support $\cand{\iterone}{i}$. 
\end{proof}   
\end{comment}


\subsection{Iterative Procedure} \label{sec; gbgic; procedure}
The iterative procedure relies on a binary tree to represent the set of candidates. We begin with a single node, the root node, which represents the set of candidates with no elements, i.e., $\candset{0}=\{\cand{0}{1}\}$, where $\cand{0}{1}=\emptyset$. 
The iterative process proceeds, with each step observing the next vertex from $j=1,\ldots,\card{\nodes}$, following the ordering specified by \eqref{eq; ordering}.
In each iterative step $j$, the following two stages are conducted: \\
\underline{\textbf{Generative stage:}} The leaves of the binary tree at level $\iterone-1$ (distant from the root node by $\iterone-1$ edges), which represent the candidates $\candset{\iterone-1}=\{\cand{\iterone-1}{1},\ldots,\cand{\iterone-1}{\card{\candset{\iterone-1}}}\}$, are split into one or two children (new leaves) according to the following rule. If leaf $i$ represents a candidate that satisfies $\cand{\iterone-1}{i}\le \sparsityterm$, it splits into two new leaves that represent: 1) $\cand{\iterone-1}{i}$; and 2) $\{\cand{\iterone-1}{i}\cup j \}$. Otherwise, the leave $i$ has only one child that represents: $\cand{\iterone-1}{i}$. 
The new leaves are stored in the set $\candset{\iterone}$, which represents the binary tree leaves in iteration $j$. Without loss of generality, the leaves are reordered from left to right. \\
\underline{\textbf{Eliminating stage:}} All of the binary search tree leaves are examined and are removed if they represent a support element $\cand{\iterone}{i}$ that satisfies 
\be \label{eq; elimination step}
\boundup{\iterone}{i}\le \gic(\leader{\iterone})
\ee
where $\boundup{\iterone}{i}$ is defined in \eqref{eq; bounding up},
and $\leader{\iterone}$ is defined as:
\be \label{eq; leader}
\leader{\iterone}=\arg\optmax{\candopt\in\candset{\iterone}} ~\gic(\candopt).
\ee
That is, we remove the candidate $\cand{\iterone}{i}\in\candset{\iterone}$ if we can prove that its upper bound is lower than the \ac{gic} of another element in $\candset{\iterone}$. 
The iterative procedure terminates in iteration $j$ when only one element is present in $j$th level of the binary tree, i.e.  
there is only one element left in $\candset{\iterone}$, and this element satisfies $\gic(\cand{\iterone}{1})=\boundup{\iterone}{1}$. 
The \ac{gbgic} method is summarized in Algorithm \ref{alg; gbgic}.
\begin{algorithm}[hbt]
\SetAlgoLined
\caption{\ac{gbgic}}
\label{alg; gbgic}
\SetKwInput{Input}{Input}
\SetKwInput{Output}{Output}
\Input{ $\measurements$, $\filter$ ,$\sparsityterm$, $\boundup{\cdot}{\cdot}$}
\Output{recovered support: $\hat{\signalsupport}$}

\BlankLine
Compute $\gic(\none)$ for $\none\in\nodes$ and order them by \eqref{eq; ordering}. \\
Initialize: $\candset{0}=\{\emptyset\}$, $\candset{\iterone}=\{~\}, ~\iterone=1,\ldots,\card{\nodes}$  \\
\For{$\iterone=1$ \KwTo $\card{\nodes}$}{
   \underline{\textbf{Generative step:}}\\
   \For{$i=1$ \KwTo $\card{\candset{\iterone-1}}$}{

       \If{$\card{\cand{\iterone-1}{i}}\le \sparsityterm$}{
        Add $\cand{\iterone-1}{i}$ and $\{\cand{\iterone-1}{i}\cup \iterone\}$ to $\candset{\iterone}$.  
       }
       \Else{Add $\cand{\iterone-1}{i}$ to $\candset{\iterone}$}
   }
   \underline{\textbf{Eliminating step:}}\\
Compute $\leader{\iterone}=\arg\optmax{\candopt\in\candset{\iterone}} ~\gic(\candopt)$\\
\For{$i=1$ \KwTo $\card{\candset{\iterone}}$}{

       \If{$\boundup{\iterone}{i}< \gic(\leader{\iterone})$}{
        Remove $\cand{\iterone}{i}$ from $\candset{\iterone}$.  
       }
   }
    \underline{\textbf{Stopping rule:}}\\
    \If{$\candset{\iterone}=1$ and $\gic(\cand{\iterone}{1})=\boundup{\iterone}{1}$}{
    \Return{$\hat{\signalsupport}=\cand{\iterone}{1}$}
    }
}

\end{algorithm}

\subsubsection{Reduce \ac{gic} Computations} \label{sec; gbgic; reduce}
In Algorithm \ref{alg; gbgic}, we can reduce the number of computations required by using an expanded representation for each leaf in the binary search tree. 
This new representation allows us to revisit the generative stage in the iterative procedure. 
In this new representation, the parent leaf represents the set ${\cand{\iterone-1}{i}}$ along with its partitions $\{\Phi_q\}_{q=1}^Q$, 
which are defined according to \eqref{eq; partition}. 
If the new leaf represents the same set as its parent leaf, then the new leaf is stored with the same partitions and the same \ac{gic} cost function. On the other hand, if the new leaf represents 
$\{\cand{\iterone-1}{i}\cup j\}$, the partitions and the \ac{gic} cost function are evaluated as follows:
\begin{itemize}
 \item If $\{j\cap \nei{2\filterdeg}{\Phi_q}\}=\emptyset$, where $\nei{2\filterdeg}{\Phi_q}$ is defined in \eqref{eq; neighborhood}, then $\Phi_q$ is copied as a subset in the new leaf.
 \item The subsets that satisfy $\{j\cap \nei{2\filterdeg}{\Phi_q}\}\ne \emptyset$ are united with each other and vertex $j$ to form one subset in the new leaf.    
\end{itemize}
It is noted that if all the subsets qualify the condition $\{j\cap \nei{2\filterdeg}{\Phi_q}\}=\emptyset$, then $j$ is added as a new subset.
The cost function of the new candidate is then computed following the linear decomposition in \eqref{eq; partition}.


\subsubsection{Discussion} \label{sec; gbgic; discussion}
The bound presented in equation \eqref{eq; bounding up} represents a more realistic assumption on the sparse recovery problem in \eqref{eq; SR 2} than the assumption made by greedy sparse recovery techniques, which often require the dictionary atoms to represent an orthogonal basis to obtain optimal results. 
Therefore, the \ac{gbgic} method is expected to have significantly more accurate support recovery performance than greedy algorithms, such as the \ac{omp} method. However, we note that in general settings the \ac{gbgic} algorithm may not converge in a reasonable amount of time. Nevertheless, when Assumptions \ref{A; graph sparse}-\ref{A; filter coefficients} hold, the algorithm is expected to perform in reasonable time. 
Specifically, it is expected to converge after a small number of iterations. 
Moreover, the number of leaves located in level $j$ of the binary tree in each iterative step $j$ is expected to remain small.

The \ac{gbgic} method is less restrictive than the \ac{gmgic} method and relies on milder assumptions. 
The main difference between the two methods is that the \ac{gbgic} method only observes a subset of the vertices in the set $\mathcal{D}$, while the \ac{gmgic} method observes all the vertices in the set $\mathcal{D}$. Moreover, the \ac{gbgic} method uses a less restrictive bound in \eqref{eq; bounding up} than the condition required in Theorem \ref{thm; partition} used in the vertex partitioning of the \ac{gmgic} method. As a result, the \ac{gbgic} method observes significantly fewer support set candidates, reducing the number of \ac{gic} computations. In conclusion, the \ac{gbgic} method provides a trade-off for the \ac{gmgic} method, as it has lower complexity but is expected to have lower support recovery performance.
Additionally, the \ac{gbgic} method can  be applied in cases where the graph filter degree is unknown.
\begin{comment}

It is assumed that the algorithm converges to a solution in a reasonable time if Assumption \ref{A; graph sparse}-\ref{A; filter coefficients} 
are satisfied.
First, it is assumed that the number of iterations until converges will be small. 
Considering Theorem \ref{thm; projection}, vertices outside the set $\nei{2\filterdeg}{\signalsupport}$ 
do not contain information on the signal and are affected only on measurement noise. 
Thus the result $\gic(\none)\le 0$ is expected for vertices $\none > \card{\nei{2\filterdeg}{\signalsupport}}$.
Moreover, considering Assumptions \ref{A; graph sparse}-\ref{A; filter degree} the number of vertices in $\nei{2\filterdeg}{\signalsupport}$
is assumed to be relatively low and significantly smaller than $\card{\{\signalsupport\in\nodes: \card{\signalsupport}\le \sparsityterm   \}}$. 
Furthermore, considering Assumption \ref{A; filter coefficients} and depending on the graphs weight and selection of \ac{gso}
the result $\gic(\none)\le \epsilon$, where $\epsilon$ represents a small value, is expected for vertices  $\none > \alpha$ where $\alpha$ is smaller than 
$\card{\nei{2\filterdeg}{\signalsupport}}$. 
Second, it is assumed that the number of elements in $\candset{\iterone}$ during the iterative procedure is maintained relatively small. 
This is due to the elimination step in the algorithm and the local behaviour dictated from Assumptions \ref{A; graph sparse}-\ref{A; filter coefficients}. 


\end{comment}

==> b_sections/d_gfoc.tex <==

\subsection{\ac{gfoc}} \label{sec; sparse; gfoc}

In this section, we introduce the \ac{gfoc} support recovery correction algorithm, which is based on Assumptions  \ref{A; graph sparse}-\ref{A; filter coefficients}. Unlike the \ac{gmgic} and \ac{gbgic} methods, \ac{gfoc} does not aim to solve the support recovery problem in \eqref{eq; gic} directly. 
Instead, it is designed to improve the accuracy of existing support recovery techniques. 
The section is organized as follows. First, we provide an overview of the method's intuition. 
Then, we present the methodology.

\subsubsection{Theory}
Consider a scenario where the support estimate is given by
\be
\hat{\signalsupport}=\{\{\signalsupport_{t}\setminus\none\}\cup \ntwo\},  
\ee
where $\ntwo\notin \signalsupport_t$. 
This estimate differs from the true support by only one vertex, and we can obtain an exact match by replacing $\none\in\signalsupport_t$ with $\ntwo\notin\signalsupport_t$. 
Given Assumptions \ref{A; graph sparse}-\ref{A; filter coefficients} and graph filter structure in \eqref{eq; graph filter}, it is highly likely that the vertices $\none$ and $\ntwo$ are neighbors in the graph $\graph$. 
So, examining each element in the support and determining whether replacing it with one of its neighbors
may be found fruitful.  
Furthermore, since every vertex in the graph is connected to a small number of neighbors, the computational complexity of this approach is expected to be low.
\subsubsection{Methodology}
The \ac{gfoc} receives as input a support set estimate provided by any support recovery algorithm, the system measurements, and the information on the underlying graph. Then, as presented in Algorithm \ref{alg; gfoc}, the \ac{gfoc} method iteratively goes over the estimated support elements and examines, for each vertex $k\in\hat{\signalsupport}$, whether replacing each element with one of the vertex in the open neighborhood set 
\be \label {eq; open neighborhood}
\firstopennei{\none}\define \{\ntwo\in\nodes: \geo{\none}{\ntwo}=1 \},
\ee
increases the \ac{gic} criterion. 
If so, it replaces the support element with its neighbor, i.e. the element in \eqref{eq; open neighborhood}, that maximizes the \ac{gic} criterion.

\begin{algorithm}[hbt]
\SetAlgoLined
\caption{\ac{gfoc}}
\label{alg; gfoc}
\SetKwInput{Input}{Input}
\SetKwInput{Output}{Output}
\Input{ $\hat{\signalsupport}$, $\graph$, $\filter$, $\measurements$}
\Output{Corrected support estimate $\hat{\signalsupport}^{c}$}

Set $\hat{\signalsupport}^c=\hat{\signalsupport}$\\ 
\For{$\none\in \hat{\signalsupport}$}{
    Compute $\hat{\ntwo}=\optmax{\ntwo\in\firstopennei{\none}} GIC(\{\hat{\signalsupport}^c\setminus\none\}\cup\ntwo)$ \\
    \If{$GIC(\{\hat{\signalsupport}^c\setminus\none\}\cup\hat{\ntwo})>GIC(\hat{\signalsupport}^c)$ }
    {
        $\signalsupport^c=\{\{\signalsupport^c\setminus \none\}\cup \hat{\ntwo}\} $
    }    
}
\Return{$\signalsupport^c$.}
\end{algorithm}
In Algorithm \ref{alg; gfoc}, the number of $\gic$ computations required is limited by $\sparsityterm d_{max}$, 
where $d_{max}$ represents the maximum degree of the graph. 
It should be noted that the output of the \ac{gfoc} method can be smaller than the input support,
as a single neighbor may replace two elements.

==> b_sections/d_gmgic.tex <==

\subsection{\ac{gmgic}} \label{sec; sparse; gmgic}

We introduce the \ac{gmgic} method in this section, which was previously presented in our earlier work [\color{red}ref\color{black}]\footnote{This conference article is yet to be published. In the meantime, should I upload the conference on Arxiv?}, for the support recovery problem in \eqref{eq; gic}.
The \ac{gmgic} method comprises four stages and builds on the assumption stated in equation \eqref{eq; order epsilon} and on Theorem \ref{thm; partition}. 
We calculate the set $\mathcal{D}$ during the first stage as defined in equation \eqref{eq; pre-screening}. In the second stage, we partition $\mathcal{D}$ into $Q$ subsets $\dsubsets$ using Algorithm \ref{alg; partition}. 
This algorithm ensures that the subsets $\dsubsets$ satisfy the condition in \eqref{eq; partition} and, thus, satisfy the decomposition in \eqref{eq; decomposition} as stated in Claim \ref{claim; partition}.
\begin{algorithm}[hbt]
\SetAlgoLined
\caption{Vertex Partitioning}
\label{alg; partition}
\SetKwInput{Input}{Input}
\SetKwInput{Output}{Output}
\Input{ $\mathcal{D}, \mathcal{V},\mathcal{E}$}
\Output{Subsets $\dsubsets$}

\BlankLine
Set $\tilde{\nodes}=\mathcal{D}$~~~ ~~~\% {\em{new graph with the vertices in $\mathcal{D}$}}\\
Set ~~~~~~~~~~~~~~~~~ \% {\em{new edge set}}
\vspace{-0.3cm}\be
\label{tilde_edge}
\tilde{\mathcal{E}}= \{(k,m):~k,m\in\hat{\mathcal{D}},~ 1\le d_{\mathcal{G}}(k,m) \le 2\Psi\}\vspace{-0.2cm}
\ee \\
Partition $\tilde{\mathcal{G}}=(\tilde{\mathcal{V}}, \tilde{\mathcal{E}})$ into its connected components (e.g., using {\em{conncomp}} command in Matlab)\\
%Set $\dsubsets$ as the vertex sets of the connected components \\
\Return{$\dsubsets$, where $\mathcal{D}_q$ includes the vertices in the $q$th component.}
\end{algorithm}
\begin{claim} \label{claim; partition}
The subsets, $\{\mathcal{D}_q\}_{q=1}^Q$, obtained from Algorithm \ref{alg; partition}, satisfy 
\eqref{eq; decomposition}.  
\end{claim}
\begin{proof}
Let $\{\mathcal{D}_q\}_{q=1}^Q$ be the subsets obtained from Algorithm \ref{alg; partition}. 
Suppose that $k$ and $m$ are in different subsets and $d_{\mathcal{G}}(k,m)<2\Psi$. 
This implies that there is an edge between these vertices in the edge set $\tilde{\mathcal{E}}$, 
i.e., $(k,m) \in \tilde{\mathcal{E}}$ ($\tilde{\edges}$ is defined in  \eqref{tilde_edge}). 
However, this contradicts our assumption since $(k,m)\in\tilde{\mathcal{E}}$ only if $k$ and $m$ are in the same connected component $\mathcal{D}_q$. 
Therefore, we can conclude that when $k$ and $m$ are in different subsets, the geodesic distance between them, i.e. $d_{\mathcal{G}}(k,m)$, is greater than $2\Psi$. 
This leads to the rule in \eqref{eq; partition}. As a result, we obtain the decomposition in \eqref{eq; decomposition}. 
\end{proof}




\begin{comment}
we reduce the dictionary 
we aim to discriminate between vertices with information on the signal $\signal$ 
and vertices that contain only noise. 
This is performed by applying a \ac{glrt} for each $m\in\mathcal{V}$ on the binary hypothesis problem:
\be
\label{H1_H0}
\begin{cases}
    \mathcal{H}_0:~\Pmat_{\{m\}}\measurements=\Pmat_{\{m\}}\filter\signal +\Pmat_{\{m\}}\nvec \\
       \mathcal{H}_1:~ \Pmat_{\{m\}}\measurements=\Pmat_{\{m\}}\nvec.
\end{cases}
\ee
The \ac{glrt} for the hypothesis testing in \eqref{H1_H0} is (p. 201 in \cite{kayfundamentals})
\vspace{-0.1cm}
\be
\label{GLRT}
\lvert \lvert \Pmat_{\filter_{\{m\}}}   \measurements \rvert\rvert^2 \mathop{\gtrless}_{\Hnull}^{\mathcal{H}_1} \rho,
\ee
where $\rho$ is a user-defined threshold.
Thus, the set $\mathcal{D}$ is estimated according to \eqref{GLRT} by 
\vspace{-0.1cm}\be  \label{eq; pre-screening 2}
\mathcal{D}\define\{m\in\mathcal{V}:~\lvert \lvert \Pmat_{\filter_{\{m\}}}   \measurements \rvert\rvert^2  >\rho\}.
\ee

In the second stage, we partition $\mathcal{D}$ by Algorithm \ref{alg; partition} into the subsets $\dsubsets$.
As shown in Claim \ref{claim; partition} these subsets satisfy 
\be \label{eq; partition 2} 
d_{\mathcal{G}}(k,m)>2\Psi,~\forall k\in\mathcal{D}q, ~~~\forall m\in\mathcal{D}{q'},
\ee
for any two subsets $\mathcal{D}_q$ and $\mathcal{D}_{q'}$  from $\{\mathcal{D}_q\}_{q=1}^Q$, where $q\ne q'$ and $1\leq Q \leq s$.
    
\end{comment}
In the third stage, we estimate the partial support set $\Omega_q$ for each subset $\mathcal{D}_q$. This set is the intersection of the support set $\Omega_t$ with $\mathcal{D}$, i.e. $\Omega_q\define\Omega_t\cap\mathcal{D}_q$. Based on \eqref{eq; gic}, 
evaluating the partial support is performed by :
\be \label{eq; gic q}
	\hat{\Omega}_q = \underset{\{\Omega\subseteq \mathcal{D}_q:~\lvert \Omega \rvert \le s\}} {\arg~\max} ~\|\Pmat_{\filter_{\Omega}}\measurements\|^2-p(\lvert \Omega \rvert).
\ee
Hence, an exhaustive search is performed locally over the vertices in $\mathcal{D}_q$. 
To compute the total support set of the sparse vector, we use the union of the partial estimates given by:
\be \label{eq; joint recovered support}
\hat{\Omega}^{temp}=\bigcup\limits_{q=1}^{Q}\hat{\Omega}_q.
\ee
In the fourth stage of the process, we correct the result from  \eqref{eq; joint recovered support} in order to ensure the sparsity restriction in \eqref{eq; sparsity restriction}. 
To do so, we first compute $\hat{\signal}_{\hat{\Omega}^{temp}}$ by substituting $\Omega=\Omega^{temp}$ into \eqref{eq; WLS}. 
Next, we select the $s$ elements from $\Omega^{temp}$ that have the highest absolute values in $\hat{\signal}_{\hat{\Omega}^{temp}}$. The algorithm for the \ac{gmgic} method is summarized in Algorithm \ref{alg; gmgic}.
\begin{algorithm}[hbt]
\SetAlgoLined
\caption{GM-GIC}
\label{alg; gmgic}
\SetKwInput{Input}{Input}
\SetKwInput{Output}{Output}
\Input{ $\measurements$, $\filter$, $\Psi$ $s$, $\rho$}
\Output{recovered support: $\hat{\Omega}$}

\BlankLine
Compute $\mathcal{D}
%\define\{m\in\mathcal{V}:~\lvert \lvert \Pmat_{\filter_{\{m\}}}   \measurements \rvert\rvert^2  >\rho_m\}.
$  from \eqref{eq; pre-screening}\\
Partition $\mathcal{D}$ by Algorithm \ref{alg; partition} to obtain
$\dsubsets$\ 

%\textbf{Multiple \ac{gic}:} \\
\For{$q=1$ \KwTo $Q$}{
    Obtain $\hat{\Omega}_q$ by \eqref{eq; gic q} \
}

Compute: $\hat{\Omega}=\bigcup\limits_{q=1}^{Q}\hat{\Omega}_q$ \

%\textbf{Sparsity Correction:} \\
\If{$|\hat{\Omega}| > s$}{
    Compute: $\signal=(\filter_{\hat\Omega}^T\filter_{\hat\Omega})^{-1}\filter^T_{\hat\Omega}\measurements$\\
    Find $\{i_1,\ldots,i_{\lvert\hat{\Omega}\rvert}\}$ such that $\lvert x_{i_{j}} \rvert \ge \lvert x_{i_{j+1}} \rvert$ \\
    Update: $\hat{\Omega}=\{i_1,\ldots,i_s\}$
}

\Return{$\hat{\Omega}$}
\end{algorithm}


==> b_sections/d_sparse.tex <==


\section{Methods for Sparse Recovery of Graph Signals} \label{Sec; theory sparse recovery}
In this section, we present three techniques for recovering a sparse graph signal from the outputs of a shift-invariant graph filter. 
These techniques, based on the analysis outlined in Subsection \ref{sec; sparse; analysis}, are introduced in the following order.
In Subsection \ref{sec; sparse; gmgic}, we introduce the \ac{gmgic} support recovery method, which involves a vertex partitioning followed by the application of the \ac{gic} criterion locally on each partitioned subset.
Next, in Subsection \ref{sec; sparse; gbgic}, we derive the \ac{gbgic} support recovery method, a binary tree search iterative approach.
Finally, in Subsection \ref{sec; sparse; gfoc}, we present the \ac{gfoc} support recovery correction method. This technique takes a support signal estimate as input and examines whether a superior solution exists within the support's local neighborhood across the graph.





==> b_sections/e_analysis.tex <==
\section{Theoretical Analysis: Recovery of Sparse Graph Signals from Graph Laplacian Excitations} \label{sec; theoretical; analysis}
In this section, we analyze the sparse recovery problem in \eqref{eq; SR 2} for the case where the dictionary matrix, $\dictionary$, is the unweighted graph Laplacian matrix, $\lap$, defined by the entries 
\be
\label{eq; unweighted laplacian}
\hspace{-0.2cm}\displaystyle L_{\none,\ntwo} = \begin{cases}
	\displaystyle \degree{\none} & \none = \ntwo \\
  \displaystyle  -1 & \edge{\none}{\ntwo} \in \edges \\
     \displaystyle 0,& \text{otherwise}
\end{cases},
\ee
where $\degree{\none}$ denotes the degree of vertex $\none$, i.e. the number of edges connected to $\none$.

The remainder of this section is organized as follows. In Subsection \ref{sec; analysis inner}, we analyze the inner product between the columns of the graph Laplacian matrix. In Subsection \ref{sec; analysis mutual}, we derive bounds on the mutual coherence of the graph Laplacian matrix. Finally, in Subsection \ref{sec; analysis projection}, we analyze the projection of the filtered signal into the single-vertex measurement subspace, presented in Theorem \ref{thm; projection}, for the case where the graph filter is a graph Laplacian matrix.

\subsection{Inner Product} \label{sec; analysis inner}
It can be verified, from \eqref{eq; unweighted laplacian}, that the inner product between two graph Laplacian matrix columns results with
\be \label{eq; inner product Laplacian}
\lap_{\none}^T\lap_{\ntwo}=\begin{cases}
\degree{\none}+\degree{\none}^2 & \none=\ntwo \\ 
 -\degree{\none}-\degree{\ntwo}+d_{in}(\none,\ntwo)& \geo{\none}{\ntwo}=1 \\
d_{in}(\none,\ntwo)   & \geo{\none}{\ntwo}=2 \\
0 & \geo{\none}{\ntwo}>2.   
\end{cases}
\ee 
where $d_{in}(\none,\ntwo)\define\card{\firstopennei{\none}\cap\firstopennei{\ntwo}}$, 
and $\firstopennei{\none}$ is defined in \eqref{eq; open neighborhood}. 
The following Claim shows that the number of shared neighbors between two vertices 
can be bounded by the minimum between the vertices degrees.  
\begin{claim} \label{thm; shared inequality min}
$
 d_{in}(\none,\ntwo)\le \min(\degree{\none},\degree{\ntwo}).     
$
\end{claim}
\begin{proof}
    We observe that $d_{in}(\none,\ntwo)$ defines the shared elements amongst 
the first order neighbors of the vertices $\none$ and $\ntwo$. 
    Thus, $d_{in}(\none,\ntwo)$ must be smaller than the number of neighbors 
    of the vertex with the minimum degree. 
\end{proof}

\begin{cor} \label{thm; shared inequality sum}
$
 2d_{in}(\none,\ntwo)\le \degree{\none}+\degree{\ntwo}.     
$
\end{cor}
\begin{proof}
$$
\begin{aligned}
 2d_{in}(\none,\ntwo)&\le 2\abs{\min(\degree{\none},\degree{\ntwo})} \\
& \le \degree{\none}+\degree{\ntwo}.     
\end{aligned}
$$
\end{proof}
\begin{cor} 
The inner product between two different graph Laplacian columns is bounded by 
\be \label{eq; inner product bound}
\abs{\lap_{\none}^T\lap_{\ntwo}}\le \degree{\none}+\degree{\ntwo}.
\ee
\end{cor}
\begin{proof}
If $\geo{\none}{\ntwo}>2$, then we obtain $\abs{\lap_{\none}^T\lap_{\ntwo}}=0\le \degree{\none}+\degree{\ntwo}$. 
If $\geo{\none}{\ntwo}=2$, then we obtain from Corollary \ref{thm; shared inequality sum} that
$\abs{\lap_{\none}^T\lap_{\ntwo}}=d_{in}(\none,\ntwo)\le 2d_{in}(\none,\ntwo)\le \degree{\none}+\degree{\ntwo}$.
Finally, if $\geo{\none}{\ntwo}=1$, then we obtain from Corollary \ref{thm; shared inequality sum} that 
$\abs{\lap_{\none}^T\lap_{\ntwo}}=\degree{\none}+\degree{\ntwo}-d_{in}(\none,\ntwo)\le \degree{\none}+\degree{\ntwo}$.
 
\end{proof}


\subsection{Mutual Coherence} \label{sec; analysis mutual}
The mutual coherence is a commonly used measure to evaluate the relationship between matrix columns in sparse recovery problems. The mutual coherence of the Laplacian matrix $\lap$ is calculated by
\be \label{eq; mutual coherence}
\mutualnot{\lap}=\optmax{\none\ne\ntwo}~\mutual{\submatcol{\lap}{\none}}{\submatcol{\lap}{\ntwo}}.
\ee
As observed, \eqref{eq; mutual coherence} takes into account the $\ell_2$ inner product between the graph Laplacian columns, which is explained in the previous section. It is important to note that the definition of mutual coherence in \eqref{eq; mutual coherence} is applicable to any matrix.

The following claim provides an upper bound to the mutual coherence of the graph Laplacian matrix:
\begin{claim} \label{thm; mutual upper}
    The mutual coherence of the unweighted graph Laplacian matrix in \eqref{eq; unweighted laplacian} can be bounded from above by
\be \label{eq; mutual upper bound L unweighted}
\mutualnot{\lap}\le \frac{2d_{\max}}{d_{\min}+d_{\min}^2}, 
\ee
where $d_{\min}$ and $d_{\max}$ denote the lowest and largest vertex degrees over the graph. 
\end{claim}
\begin{proof}
By substituting \eqref{eq; inner product bound} in \eqref{eq; mutual coherence} and using the results in \eqref{eq; inner product Laplacian} for $k=m$,
we obtain
\be \label{eq; mutual Laplacian upper bound}
\begin{aligned}
\mutualnot{\lap} &\le \optmax{\none\ne\ntwo}\frac{\degree{\none}+\degree{\ntwo}}{\sqrt{\degree{\none}+\degree{\none}^2 }\sqrt{\degree{\ntwo}+\degree{\ntwo}^2 }} \\
&\le \frac{2d_{\max}}{d_{\min}+d_{\min}^2}.
\end{aligned}
\ee
\end{proof}
The following claim provides a lower bound to the mutual coherence of the graph Laplacian matrix:
\begin{claim} \label{thm; mutual lower}
The mutual coherence of the unweighted graph Laplacian matrix in \eqref{eq; unweighted laplacian} can be bounded from below by
\be \label{eq; mutual lower bound L unweighted}
\mutualnot{\lap}\ge \frac{d_{\min}}{d_{\max}+d_{\max}^2}, 
\ee
where $d_{\min}$ and $d_{\max}$ denote the lowest and largest vertex degrees over the graph.
\end{claim}
\begin{proof}
   Case 1: The mutual coherence is obtained between nodes $\none$ and $\ntwo$ that satisfy $\geo{\none}{\ntwo}=1$. 
   In this case and based on Claim \ref{thm; shared inequality min}, we obtain:
    \be \label{eq; mutual upper}
    \begin{aligned}
        \mutualnot{\lap}&=\frac{\degree{\none}+\degree{\ntwo}-d_{in}(\none,\ntwo)}
        {\sqrt{\degree{\none}+\degree{\none}^2 }\sqrt{\degree{\ntwo}+\degree{\ntwo}^2 }} \\
        &\ge  \frac{\degree{\none}+\degree{\ntwo}-\min(\degree{\none},\degree{\ntwo})}
        {\sqrt{\degree{\none}+\degree{\none}^2 }\sqrt{\degree{\ntwo}+\degree{\ntwo}^2 }} \\
        &=  \frac{\max(\degree{\none},\degree{\ntwo})}
        {\sqrt{\degree{\none}+\degree{\none}^2 }\sqrt{\degree{\ntwo}+\degree{\ntwo}^2 }} \\
        &\ge  \frac{d_{min}}
        {d_{\max}+d_{\max}^2} 
    \end{aligned}
    \ee
Case 2: The mutual coherence is obtained between nodes $\none'$ and $\ntwo'$ that satisfy $\geo{\none'}{\ntwo'}=2$. 
 However, in that case, $k$ and $m$ exist, such as $\geo{\none}{\ntwo}=1$ that do not maximize the mutual coherence. 
 Hence, the mutual coherence is larger or equal to the results obtained by substituting $\none$ and $\ntwo$ in the component in the maximization in \eqref{eq; mutual coherence}. 
 Therefore, we get the same result in \eqref{eq; mutual upper} while replacing the $=$ with $\ge$ in the first line. 
\end{proof}

As a special case, we consider $d$-regular graphs in which the vertex degree is equal over the graph. 
In this case, by substituting $d=d_{\min}=d_{\max}$ in \eqref{eq; mutual upper bound L unweighted} and \eqref{eq; mutual lower bound L unweighted},
we obtain that the mutual coherence of the unweighted Laplacian matrix
can be bounded by 
\be \label{eq; mutual bound L unweighted regular}
\frac{1}{1+d} \le \mutualnot{\lap}\le \frac{2}{1+d}.
\ee
As observed in \eqref{eq; mutual bound L unweighted regular}, the mutual coherence of $d$-regular graphs is not affected by the size of the model. 
However, it does decrease as the vertex degree of the graph increases. 
Therefore, if the graph has a high degree, distinguishing between dictionary atoms becomes easier.


\subsection{Projection into a Single-vertex Measurement Subspace} \label{sec; analysis projection}
In Theorem \ref{thm; projection}, we demonstrated that the projection over a measurement space that consists of a single vertex is only non-zero if the vertex is located within the closed $2\filterdeg$-order neighborhood, of the signal support, which is defined in \eqref{eq; neighborhood}. 
Therefore, for the unweighted graph Laplacian, where the filter degree equals one, we obtain that
$$
\projlap{\ntwo}\lap_{\none}\signalentry_\none=\zerovec, 
$$ 
when $\geo{\none}{\ntwo}>2$. 
Additionally, the next claim suggests that the projection decreases with respect to its distance from the sparse signal locations.

\begin{claim} \label{thm; projection decreases}
If $\geo{\none}{\ntwo}<\geo{\iterone}{\ntwo}$ then
\be \label{eq; projection order}
\norm{\Pmat_{\lap_{\ntwo}}\lap_{\none}}^2\ge
\norm{\Pmat_{\lap_{\ntwo}}\lap_{\iterone}}^2 
\ee
\end{claim}
\begin{proof}
If $\none=\ntwo$, then from projection properties, we obtain that 
\eqref{eq; projection order} is true for any selection of $\iterone\ne \none$ (see Theorem 2.22 on page 46 in \cite{yanai2011projection}). 
If $\geo{\ntwo}{\none}=1$ then evidently \eqref{eq; projection order} 
is true if $\geo{\ntwo}{\iterone}>2$ where in that case the r.h.s. equals zero. 
If $\geo{\ntwo}{\iterone}=2$ then by Claim \ref{thm; shared inequality min} we obtain:
$$
\begin{aligned}
\norm{\Pmat_{\lap_{\ntwo}}\lap_{\iterone}}^2&\underset{a}{=} \norm{\lap_{\ntwo}}^2\frac{\lap_{\ntwo}^T\lap_{\iterone}}{\norm{\lap_{\ntwo}}^2}\\
&\underset{b}{=} \norm{\lap_{\ntwo}}^2\frac{d_{in}(\ntwo,\iterone)}{\norm{\lap_{\ntwo}}^2}\\
&\underset{c}{\le}  \norm{\lap_{\ntwo}}^2\frac{\min(\degree{\ntwo},\degree{\iterone})}{\norm{\lap_{\ntwo}}^2}\\
%&\underset{d}{\le}  \norm{\lap_{\ntwo}}^2\frac{\degree{\ntwo}}{\norm{\lap_{\ntwo}}^2} \\
%&\le \norm{\lap_{\ntwo}}^2\frac{\max(\degree{\none},\degree{\ntwo})}{\norm{\lap_{\ntwo}}^2} \\
%&= \norm{\lap_{\ntwo}}^2\frac{\degree{\none}+\degree{\ntwo}-\min(\degree{\none},\degree{\ntwo})}{\norm{\lap_{\ntwo}}^2} \\
&\underset{d}{\le}   \norm{\lap_{\ntwo}}^2\frac{\degree{\ntwo}+\degree{\none}-d_{in}(\none,\ntwo)}{\norm{\lap_{\ntwo}}^2} \\
&\underset{e}{=} \norm{\lap_{\ntwo}}^2\frac{\lap_{\ntwo}^T\lap_{\none}}{\norm{\lap_{\ntwo}}^2}=\norm{\Pmat_{\lap_{\ntwo}}\lap_{\none}}^2.
\end{aligned}
$$
It is noted that Claim \ref{thm; shared inequality min} is used in the transition between 
lines $b$ and $c$ and in the transition between lines $c$ and $d$. 
\end{proof}
Claim \ref{thm; projection decreases} asserts that the projection of the filtered signal $\filter\signal$ onto single-vertex measurements strictly decreases with the distance from vertices in the signal support $\signalsupport$. 
In other words, the further a vertex is from the vertices included in the sparse signal support set, the less information it provides about the filtered signal.


%=======================================================================================
%                                           Graveyard                                   %
%=======================================================================================
%=======================================================================================
%=======================================================================================
%=======================================================================================
%=======================================================================================

\begin{comment}
{\renewcommand{\arraystretch}{1.2} %<- modify value to suit your needs

\begin{table} [h!]
\centering
\begin{tabular}{c|c|c|c|c}  
~ & \multicolumn{2}{c|}{\textbf{$2$-regular graph}} & \multicolumn{2}{c}{\textbf{$4$-regular graph}} \\  \hline 
\underline{$\geo{\none}{\ntwo}$}  & \underline{$\lap_{\none}^T\lap_{\ntwo}$} & \underline{$\norm{\Pmat_{\lap_{\ntwo}}\lap_{\none}}^2$} & \underline{$\lap_{\none}^T\lap_{\ntwo}$} 
&\underline{$\norm{\Pmat_{\lap_{\ntwo}}\lap_{\none}}^2$} \\
$0$ & $6$ & $6$ & $20$ &$20$  \\
$1$ & $-4$ & $0.6667$   & -8 & $0.4$        \\
$2$ & $1$ & $0.1667$ & 1 & $0.05$ \\
$>2$ & $0$ & $0$  & $0$ & $0$
\end{tabular}
\caption{The inner product and single space projection for $\lap$.}
\label{table; Laplacian}
\end{table}

\end{comment}

\begin{comment}


\subsection{Support estimation problem}


\subsection{Analysis}
%\begin{rem}
%    Any subset of the graph filter columns is linearly independend. 
%\end{rem}
Orthogonality condition between $2$ graph filter columns 
\begin{thm} \label{thm; ortho two columns}
   Orthogonality condition between two graph filter columns: 
\renewcommand{\puneq}{}\loadeq{FilterOrthogonalityCondition} 
\end{thm}
\begin{proof}
 \loadeq{FilterEntryCondition}
 \color{red} complete the proof \\
 I think this comes later when reducing the number of measurements \color{black}
\end{proof}

\subsubsection{Single-vertex measurement subspace}

Assume that the true support of $\xvec$ is $\Omega_t$. % is known.  
In this case, taking into account that $x_k=0$ for any $k\notin \Omega_t$, the filtered signal %$\Fmat\xvec=\sum\limits_{k\in\mathcal{V}} \Fmat_{k}x_k$
satisfies
\be \label{eq; filtered signal}
\Fmat\xvec=\Fmat_{\Omega_t}\xvec_{\Omega_t}=\sum\limits_{k\in\Omega_t} \Fmat_{\{k\}}x_k. 
\ee
In addition, we define the $2\Psi$ neighborhood of $\Omega_t$ as 
\be \label{eq; A set}
\mathcal{N}_{2\Psi}(\Omega_t)\define\{m\in\mathcal{V}:~\exists k\in\Omega_t~\text{s.t.}~0\le d_{\mathcal{G}}(k,m)\le 2\Psi\},
\ee
which leads to the following theorem.


\begin{thm}\label{thm; projection}
 The projection of the filtered signal on the single-vertex measurement subspace $\text{col}(\Fmat_{m})$ satisfies
\be \label{eq; filtered 0}
\Pmat_{\Fmat_{\{m\}}}\Fmat\xvec=\Pmat_{\Fmat_{\{m\}}}\Fmat_{\Omega_t}\xvec_{\Omega_t}=\zerovec,
~~~\forall
m\notin \mathcal{N}_{2\Psi}(\Omega_t).
\ee
\end{thm}
\begin{proof}
 If the geodesic distance between vertices $k$ and $m$, $d_{\mathcal{G}}(k,m)$, is larger than $2\Psi$,  then 
\eqref{eq; F prop 2}  and the definition of projection matrix imply that
%the projection of the component $\Fmat_{k}x_k$ on the single-vertex measurement subspace $\text{col}(\Fmat_{m})$ satisfies
\be \label{eq; 2nd 0}
\begin{aligned}
\Pmat_{\Fmat_{\{m\}}}\Fmat_{\{k\}}
=\Fmat_m(\Fmat_m^T\Fmat_m)^{-1}\Fmat^T_m\Fmat_k  = \zerovec,
\end{aligned}
\ee
where $\Fmat_{\{k\}}$ is the $k$th column of $\Fmat$, and $\Pmat_{\Fmat_{\{m\}}}$ is
the projection matrix onto the single-column space $\text{col}(\Fmat_{m})$.
 Multiplying \eqref{eq; filtered signal} by $\Pmat_{\Fmat_{\{m\}}}$, $m\notin \mathcal{N}_{2\Psi}(\Omega_t)$,
and substituting \eqref{eq; 2nd 0}, results in \eqref{eq; filtered 0}.  
\end{proof}

\begin{rem}
Depending on the edge weights of the graph $\{\edgeweight_{\none}\}_{\none}$ and considering Assumption \ref{A; filter coefficients}, there exists a set $\candidateset\subset\nei{2\filterdeg}{\signalsupport_{t}}$
such that 
\be \label{eq; D}
\|\Pmat_{\Fmat_{\{m\}}}\Fmat_{\Omega_t}\xvec_{\Omega_t}\|_2^2<\epsilon,~~~\forall m\in\{\mathcal{N}_{2\Psi}(\Omega_t)\setminus\mathcal{D}\},
\ee 
where $\epsilon$ is  small.
\end{rem}
\color{red} maybe add a norm to $\signal$.  or normalize by $\signal$ \color{black}

\begin{thm}
Consider an unweighted graph with $\signalsupport=\none$ and define the graph filter as $\Fmat=\lap$. 
If $\geo{\none}{\ntwo}\le \geo{\none}{\iterone}$, then 
\be
\norm{\proj{\ntwo}{\filter\signal}}\ge \norm{\proj{\iterone}\filter\signal}
\ee
    
\end{thm}

\begin{rem}
It is likely that the signal support set, $\signalsupport_t$, is located in the set $\candidateset$. 
\end{rem}
\color{red} show for random signal \\
\color{black}
%We denote the \ac{gic} cost function by 
%\renewcommand{\puneq}{ }\loadeq{gicfunc}
Without loss of generality we assume that the vertices of the graph are ordered such that
\renewcommand{\puneq}{ }\loadeq{order}
\begin{rem}
It is likely that the vertices located in the set $\candidateset$ and particularly the ones in $\signalsupport_{t}$ 
are the ones starting the list of vertices ordered by \eqref{eq; order}. 
\end{rem}
\begin{rem}
If $\Omega_t=k$ then $\gic(k)$ is the maximum. 
\end{rem}



\subsubsection{Multiple-vertec measurement subspace}
\begin{hip}
Let $\signalsupport_t=\signalsupport_{1}\cup \none$.
In addition, satisfy $\gic(\none)\le\gic(\iterone)$, where $\iterone\in\signalsupport$
and $\signalsupport=\signalsupport_1\cup\ntwo$ such that $\signalsupport_1\subseteq\signalsupport_{t}$ 
yet $\ntwo\notin \signalsupport_{t}$. Then, it is likely that  
\be \label{eq; mult analysis}
\gic(\signalsupport)\le \gic(\signalsupport_{1})+\gic(\none). 
\ee
\end{hip}
Discussion:  \\
The vertex $\ntwo$ is a noise vertex where $\ntwo\notin \signalsupport_{m}$. 
Hence, we should consider three cases:
\begin{enumerate}
\item \textbf{Case 1 ($\Pmat_{\Fmat_{\{m\}}}\Fmat_{\signalsupport_{1}}=0$, $\Pmat_{\Fmat_{\{\ntwo\}}}\Fmat_{\{\none\}}\ne 0$):}
If this is the case it is $\gic(\none)\le\gic(\ntwo)$. 
\item  \textbf{Case 2 ($\Pmat_{\Fmat_{\{m\}}}\Fmat_{\signalsupport_{1}}\ne 0$, $\Pmat_{\Fmat_{\{\ntwo\}}}\Fmat_{\{\none\}}= 0$):}
If this is the case we obtain that $\gic(\signalsupport)\ge \gic(\signalsupport_1)$ and thus it is likely that the 
result in \eqref{eq; mult analysis} is obtained. 
\item  \textbf{Case 3 ($\Pmat_{\Fmat_{\{m\}}}\Fmat_{\signalsupport_{1}}\ne 0$, $\Pmat_{\Fmat_{\{\ntwo\}}}\Fmat_{\{\none\}}\ne 0$):}
Assumption \ref{A; graph sparse}-\ref{A; filter coefficients} define a unique structure to the graph 
that propogates to the structure of the graph filter through \eqref{eq; graph filter}
when selecting the \ac{gso} as the graph Laplacian matrix in \eqref{eq; graph laplacian}. 
\end{enumerate}

\begin{figure}[hbt]
\centering
 \includegraphics[width=4cm]{a_figures/example_mult.png}
 \caption{Example}
\label{fig; example multiple}
\end{figure}
 Consider the following example in Fig. \ref{fig; example multiple} for the setting that $\gso=\lap$
 and $\filterdeg=1$. 
 In this case, it is probable that $\gic(\ntwo)\ge \gic(\none)$ becuase it could be affected by 
 the two sources: 1) the one originating from $\none$; and 2) the one originating from $\signalsupport_1$. 
 The filtered signal $\filter\signal$ non zero entries are located in $\nei{1}{\signalsupport_t}=\{2,3,4,5,7,8,10,11,12,13,14,15\}$. 

In the following we explain why including $\ntwo$ in the support instead of $\none$ provides a poor representation 
promoting the result in \eqref{eq; mult analysis}. 
Considering the properties from \eqref{eq; gso} the measurements in $\{13,14,15\}$ are not considered in 
the measurement space $\text{col}(\Omega_1\cup \ntwo)$. 
Second, the zero measurement in $\{6\}$ is nonzero if $\ntwo$ is considered part of the signal support. 
Third, one of the following two cases must occur: 1) the measurements in $\{10,12\}$ are represented with opposite 
sign when compared to their representation by $\text{col}(\filtercolumn{\none})$; 
or 2) the measurement in $\{11\}$ is represented with opposite sign when compared to the representation by 
$\text{col}(\filtercolumn{\none})$. 
Fourth, in order to properly represent the measurement in $\none$ the signal value in $\ntwo$ must be significanlty 
larger then the true value of the signal in the location $\none$. 

\color{red} 
Comments:
\begin{itemize}
    \item How can we use this knowledge in order to better explain case 3. 
    \item This, in addition to the signle-vertex measurement subspace analysis is the basis for our method. 
    \item We can consider explaining other cases. 
    \item generalization for this result: 1) to a higher graph degree; 2) switch single nodes $(\none,\ntwo)$ with subsets. 
\end{itemize}


\color{black}

\end{comment} 


\begin{comment}
\subsection{Inner product} \label{sec; analysis inner}
\color{red} The weighted case is more complicated then what I thought. 
\color{black}

The weighted graph Laplacian, $\lap$, is defined by the entries
\be \label{eq; weighted Laplacian}
\displaystyle L_{\none,\ntwo} = \begin{cases}
	\displaystyle \degree{\none} & \none = \ntwo \\
  \displaystyle  -\edgeweight_{\none,\ntwo} & \edge{\none}{\ntwo} \in \edges \\
     \displaystyle 0,& \text{otherwise}
\end{cases},
\ee
where 
\be \label{eq; degree weighted}
\degree{\none}=\sum_{\iterone\in\nodes} \indicator{\{\geo{\none}{\iterone}=1\}} \edgeweight_{\none,\iterone}. 
 \ee
It can be verified, from \eqref{eq; weighted Laplacian}, that the inner product between two graph Laplacian matrix columns is given by 
\be \label{eq; inner product Laplacian}
\lap_{\none}^T\lap_{\ntwo}=\begin{cases}
\degree{\none}+\degree{\none}^2 & \none=\ntwo \\ 
 -\degree{\none}-\degree{\ntwo}+d_{in}(\none,\ntwo)& \geo{\none}{\ntwo}=1 \\
d_{in}(\none,\ntwo)   & \geo{\none}{\ntwo}=2 \\
0 & \geo{\none}{\ntwo}>2,  
\end{cases}
\ee 
where
$$
d_{in}(\none,\ntwo)=\sum_{\iterone\in\nodes} \indicator{\{\geo{\none}{\iterone}=1,\geo{\ntwo}{\iterone}=1\}}\edgeweight_{\ntwo,\iterone}.
 $$
\begin{claim} \label{thm; shared inequality}
 If the edge weights in \eqref{eq; weighted Laplacian} are smaller or equal than $1$, 
 then Claims \ref{thm; shared inequality}-\ref{thm; mutual lower} are also true
 for the weighted graph Laplacian. 
\end{claim}
\begin{proof}
The edge weights are smaller or equal to one. Therefore
$$
\begin{aligned}
d_{in}(\none,\ntwo)&=\sum_{\iterone\in\nodes} \indicator{\{\geo{\none}{\iterone}=1,\geo{\ntwo}{\iterone}=1\}}_{\none,\iterone}\edgeweight_{\ntwo,\iterone}  \\
&\le \sum_{\iterone\in\nodes} \indicator{\{\geo{\none}{\iterone}=1,\geo{\ntwo}{\iterone}=1\}}\edgeweight_{\none,\iterone} \\
&\le \sum_{\iterone\in\nodes} \indicator{\{\geo{\none}{\iterone}=1\}} \edgeweight_{\none,\iterone} \\
&=\degree{\none}. 
\end{aligned}
$$
\end{proof}


\subsection{Mutual Coherence} \label{sec; analysis mutual}
\color{red} relate our results to known mutual coherence results \color{black}. 
 In this subsection, we study the mutual coherence of the graph Laplacian matrix.
\renewcommand{\puneq}{,} \loadeq{MutualDef} 
takes into account the $\ell_2$ inner product between the graph Laplacian columns.

The following theorems provide upper and lower bounds on the mutual coherence: 



\begin{claim} \label{thm; mutual lower}
The mutual coherence of the unweighted graph Laplacian matrix in \eqref{eq; unweighted laplacian} can be bounded from below by
\be \label{eq; mutual lower bound L unweighted}
\mutualnot{\lap}\le \frac{2d_{\min}}{d_{\max}+d_{\max}^2}, 
\ee
where $d_{\min}$ and $d_{\max}$ denote the lowest vertex degree and the largest vertex degree over the graph. 
\end{claim}
\begin{proof}
   Case 1: The mutual coherence is obtained between nodes $\none$ and $\ntwo$ that satisfy $\geo{\none}{\ntwo}=1$. 
   In that case, we obtain:
    \be \label{eq; mutual upper}
    \begin{aligned}
        \mutualnot{\lap}&=\frac{\degree{\none}+\degree{\ntwo}-d_{in}(\none,\ntwo)}
        {\sqrt{\degree{\none}+\degree{\none}^2 }\sqrt{\degree{\ntwo}+\degree{\ntwo}^2 }} \\
        &\ge  \frac{\degree{\none}+\degree{\ntwo}}
        {\sqrt{\degree{\none}+\degree{\none}^2 }\sqrt{\degree{\ntwo}+\degree{\ntwo}^2 }} \\
        &\ge  \frac{2d_{min}}
        {d_{\max}+d_{\max}^2} 
    \end{aligned}
    \ee
Case 2: The mutual coherence is obtained between nodes $\none'$ and $\ntwo'$ that satisfy $\geo{\none'}{\ntwo'}=2$. 
 However, in that case, there exists $k$ and $m$ such that $\geo{\none}{\ntwo}=1$ that do not maximize the mutual coherence. 
 Therefore, we get the same result in \eqref{eq; mutual upper} while replacing the $=$ with $\ge$ in the first line. 

\end{proof}
As a special, we consider $d$-regular graphs in which the vertex degree is equal over the graph. 
In this case, by substituting $d=d_{\min}=d_{\max}$ in \eqref{eq; mutual upper bound L unweighted} and \eqref{eq; mutual lower bound L unweighted},
we obtain that the mutual coherent of the unweighted Laplacian matrix
is given by 
\be \label{eq; mutual bound L unweighted regular}
 \mutualnot{\lap}= \frac{2}{1+d}.
\ee
Hence, the mutual coherence of $d$-regular graphs decreases with the increase of the graph vertex degree. 


\end{comment}


\begin{comment}

For simplicity, we first show our results for the unweighted graph Laplacian matrix, $\lap$, 
which is defined by the entries 
\be
\label{eq; unweighted laplacian}
\hspace{-0.2cm}\displaystyle L_{\none,\ntwo} = \begin{cases}
	\displaystyle \degree{\none} & \none = \ntwo \\
  \displaystyle  -1 & \edge{\none}{\ntwo} \in \edges \\
     \displaystyle 0,& \text{otherwise}
\end{cases},
\ee
where $\degree{\none}$ is the $\none$ vertex degree, i.e. number of neighbors. 
Then, if possible, we generalize the results also for the weighted graph Laplacian, $\lap^{\edgeweight}$, which is defined by the entries
\be \label{eq; weighted Laplacian}
\displaystyle L^{\edgeweight}_{\none,\ntwo} = \begin{cases}
	\displaystyle \degree{\none}^{\edgeweight} & \none = \ntwo \\
  \displaystyle  -\edgeweight_{\none,\ntwo} & \edge{\none}{\ntwo} \in \edges \\
     \displaystyle 0,& \text{otherwise}
\end{cases},
\ee
where 
\be \label{eq; degree weighted}
\degree{\none}^{\edgeweight}=\sum_{\iterone\in\nodes} \indicator{\{\geo{\none}{\iterone}=1\}} \edgeweight_{\none,\iterone}. 
 \ee
In Subsection \ref{sec; analysis mutual}, we derive bounds for the graph Laplacian matrix mutual coherence [ref].
Then, in Subsection \ref{sec; analysis projection} we study the single-vertex measurement subspace of the graph Laplacian matrix, 
as defined in \eqref{eq; filtered 0}. 
 


\subsection{Mutual Coherence} \label{sec; analysis mutual}
\color{red} relate our results to known mutual coherence results \color{black}. 
 In this subsection, we study the mutual coherence of the graph Laplacian matrix.
\renewcommand{\puneq}{,} \loadeq{MutualDef} 
takes into account the $\ell_2$ inner product between the graph Laplacian columns.
It can be verified, from \eqref{eq; unweighted laplacian}, that the inner product between two graph Laplacian matrix columns is given by 
\be \label{eq; inner product Laplacian}
\lap_{\none}^T\lap_{\ntwo}=\begin{cases}
\degree{\none}+\degree{\none}^2 & \none=\ntwo \\ 
 -\degree{\none}-\degree{\ntwo}+d_{in}(\none,\ntwo)& \geo{\none}{\ntwo}=1 \\
d_{in}(\none,\ntwo)   & \geo{\none}{\ntwo}=2 \\
0 & \geo{\none}{\ntwo}>2.   
\end{cases}
\ee 
where $d_{in}(\none,\ntwo)\define\card{\firstopennei{\none}\cap\firstopennei{\ntwo}}$. 

The following theorems provide upper and lower bounds on the mutual coherence: 
\begin{claim} \label{thm; shared inequality}
$
 2d_{in}(\none,\ntwo)\le \degree{\none}+\degree{\ntwo}.     
$
\end{claim}
\begin{proof}
    First, we observe that $d_{in}(\none,\ntwo)$ define the shared elements amongst 
the first order neighbors of the vertices $\none$ and $\ntwo$. 
Thus, this number must be lower then the minimal degree between $\none$ and $\ntwo$. 
Consequently, we obtain that
$$
\begin{aligned}
 2d_{in}(\none,\ntwo)&\le 2\abs{\min(\degree{\none},\degree{\ntwo})} \\
& \le \degree{\none}+\degree{\ntwo}.     
\end{aligned}
$$
\end{proof}

\begin{claim} \label{thm; mutual upper}
    The mutual coherence of the unweighted graph Laplacian matrix in \eqref{eq; unweighted laplacian} can be bounded from above by
\be \label{eq; mutual upper bound L unweighted}
\mutualnot{\lap}\le \frac{2d_{\max}}{d_{\min}+d_{\min}^2}, 
\ee
where $d_{\min}$ and $d_{\max}$ denote the lowest vertex degree and the largest vertex degree over the graph. 
\end{claim}
\begin{proof}
Based on Claim \ref{thm; shared inequality},
we can bound the inner product in \eqref{eq; inner product Laplacian} by
\be \label{eq; inner upper bound}
\abs{\lap_{\none}^T\lap_{\ntwo}}\le \degree{\none}+\degree{\ntwo}.
\ee
Notice that this result applies both for $\geo{\none}{\ntwo}=1$ and $\geo{\none}{\ntwo}=2$.
By substituting \eqref{eq; inner upper bound} in \eqref{eq; mutual coherence}, 
we obtain
\be \label{eq; mutual Laplacian upper bound}
\begin{aligned}
\mutualnot{\lap} &\le \optmax{\none\ne\ntwo}\frac{\degree{\none}+\degree{\ntwo}}{\sqrt{\degree{\none}+\degree{\none}^2 }\sqrt{\degree{\ntwo}+\degree{\ntwo}^2 }} \\
&\le \frac{2d_{\max}}{d_{\min}+d_{\min}^2}.
\end{aligned}
\ee
\end{proof}

\begin{claim} \label{thm; mutual lower}
The mutual coherence of the unweighted graph Laplacian matrix in \eqref{eq; unweighted laplacian} can be bounded from below by
\be \label{eq; mutual lower bound L unweighted}
\mutualnot{\lap}\le \frac{2d_{\min}}{d_{\max}+d_{\max}^2}, 
\ee
where $d_{\min}$ and $d_{\max}$ denote the lowest vertex degree and the largest vertex degree over the graph. 
\end{claim}
\begin{proof}
   Case 1: The mutual coherence is obtained between nodes $\none$ and $\ntwo$ that satisfy $\geo{\none}{\ntwo}=1$. 
   In that case, we obtain:
    \be \label{eq; mutual upper}
    \begin{aligned}
        \mutualnot{\lap}&=\frac{\degree{\none}+\degree{\ntwo}-d_{in}(\none,\ntwo)}
        {\sqrt{\degree{\none}+\degree{\none}^2 }\sqrt{\degree{\ntwo}+\degree{\ntwo}^2 }} \\
        &\ge  \frac{\degree{\none}+\degree{\ntwo}}
        {\sqrt{\degree{\none}+\degree{\none}^2 }\sqrt{\degree{\ntwo}+\degree{\ntwo}^2 }} \\
        &\ge  \frac{2d_{min}}
        {d_{\max}+d_{\max}^2} 
    \end{aligned}
    \ee
Case 2: The mutual coherence is obtained between nodes $\none'$ and $\ntwo'$ that satisfy $\geo{\none'}{\ntwo'}=2$. 
 However, in that case, there exists $k$ and $m$ such that $\geo{\none}{\ntwo}=1$ that do not maximize the mutual coherence. 
 Therefore, we get the same result in \eqref{eq; mutual upper} while replacing the $=$ with $\ge$ in the first line. 

\end{proof}
As a special, we consider $d$-regular graphs in which the vertex degree is equal over the graph. 
In this case, by substituting $d=d_{\min}=d_{\max}$ in \eqref{eq; mutual upper bound L unweighted} and \eqref{eq; mutual lower bound L unweighted},
we obtain that the mutual coherent of the unweighted Laplacian matrix
is given by 
\be \label{eq; mutual bound L unweighted regular}
 \mutualnot{\lap}= \frac{2}{1+d}.
\ee
Hence, the mutual coherence of $d$-regular graphs decreases with the increase of the graph vertex degree. 

The weighted graph Laplacian matrix is provided in \eqref{eq; weighted Laplacian}. 
It can be verified that the inner product of the weighted graph Laplacian is similar to the one in \eqref{eq; inner product Laplacian}
when substituting $\degree{\none}^{\edgeweight}$ from \eqref{eq; degree weighted} and 
$$
d_{in}^{\edgeweight}(\none,\ntwo)=\sum_{\iterone\in\nodes} \indicator{\{\geo{\none}{\iterone}=1,\geo{\ntwo}{\iterone}=1\}} \edgeweight_{\none,\iterone}\edgeweight_{\ntwo,\iterone}.
 $$
\begin{claim}
 If the edge weights in \eqref{eq; weighted Laplacian} are smaller or equal than $1$, 
 then Claims \ref{thm; shared inequality}-\ref{thm; mutual lower} are also true
 for the weighted graph Laplacian. 
\end{claim}
\begin{proof}
The edge weights are smaller or equal to one. Therefore
$$
\begin{aligned}
d_{in}^{\edgeweight}(\none,\ntwo)&=\sum_{\iterone\in\nodes} \indicator{\{\geo{\none}{\iterone}=1,\geo{\ntwo}{\iterone}=1\}} \edgeweight_{\none,\iterone}\edgeweight_{\ntwo,\iterone}  \\
&\le \sum_{\iterone\in\nodes} \indicator{\{\geo{\none}{\iterone}=1,\geo{\ntwo}{\iterone}=1\}} \edgeweight_{\none,\iterone} \\
&\le \sum_{\iterone\in\nodes} \indicator{\{\geo{\none}{\iterone}=1\}} \edgeweight_{\none,\iterone} \\
&=\degree{\none}^{\edgeweight}. 
\end{alinged}
$$
Following the same step we obtain that $d_{in}^{\edgeweight}(\none,\ntwo)\le \degree{\ntwo}^{\edgeweight}$. 
As a result we optain that $2d_{in}^{\edgeweight}(\none,\ntwo)\le \degree{\none}^{\edgeweight}+\degree{\ntwo}^{\edgeweight}$, 
and, thus, Claim \ref{thm; shared inequality} is maintained. 
Moreover, Claim \ref{thm; shared inequality} is the basis for the proofs of both Claims \ref{thm; mutual upper}-\ref{thm; mutual lower}, 
and, thus, they are also maintained. 
\end{proof}

\end{commennt}

\begin{comment}
  \begin{thm}
If the maximal degree satisfies, $d_{\max}\le 6$, then 
\be \label{eq; mutual bound L unweighted degree}
\frac{1}{6}\le \mutualnot{\lap}
\ee
and the vertices that maximize the mutual coherence, i.e. $\none$ and $\ntwo$ that maximize \eqref{eq; mutual coherence}, are neighbors, 
i.e. $\geo{\none}{\ntwo}=1$
\end{thm}
\begin{proof} 
Add proof. \color{red} It could be a pickle. 
Now, the proof is half numerical. Check with Tirza what she thinks about proving something this way. \color{black} 
\end{proof}  

\begin{thm}
The mutual coherence of the Laplacian matrix in \eqref{eq; unweighted laplacian}
for a $2$-regular graph is: 

\be \label{eq; mutual Laplacian 2 regular}
\mutualnot{\lap}=\frac{2}{3}
\ee       
\end{thm}
\begin{proof}
\color{red}Use Table \ref{table; Laplacian}.  \color{black}
\end{proof}


\begin{thm}
The mutual coherence of the Laplacian matrix in \eqref{eq; unweighted laplacian}
for a $4$-regular graph is: 
\be \label{eq; mutual Laplacian 4 regular}
   \mutualnot{\lap}=\frac{2}{5}
    \ee    
\end{thm}
\begin{proof}
\color{red} Use Table \ref{table; Laplacian}. \color{black}  
\end{proof}

\begin{rem}
    The vertices that maximize the mutual coherence in \eqref{eq; mutual Laplacian 2 regular}
    and \eqref{eq; mutual Laplacian 4 regular} are neighbors.
\end{rem}

\end{comment}

==> b_sections/g_simulations.tex <==
\section{Performance Evaluation} \label{sec; simulations}

In this section, we present a performance evaluation of the proposed algorithms. We illustrate the simulation setup in Subsection \ref{sec; sim; set up}. Subsequently, in Subsection \ref{sec; sim; F-score}, we demonstrate the superiority of the proposed methods over the \ac{omp} and Lasso methods in terms of support recovery performance. Finally, in Subsection \ref{sec; sim; run}, we exhibit the efficiency of the proposed methods and show that they run competitively compared to the \ac{omp} and Lasso methods. The results are presented over two different frameworks: 1) a $2$D-graph with $100$ vertices as shown in Fig. \ref{fig; 2D}; and 2) a realization of the Erd\H{o}s-R\'enyi graph with $70$ vertices as shown in Fig. \ref{fig; erdos}.

\subsection{Set Up} \label{sec; sim; set up}

\subsubsection{Model}

The problem of support recovery in \eqref{eq; sup} is considered with the graph filter, $\filter$, in \eqref{eq; graph filter} as the dictionary matrix, and the weighted graph Laplacian matrix\footnote{The weighted graph Laplacian is a generalization of the unweighted Laplacian matrix in \eqref{eq; unweighted laplacian}. The weighted Laplacian matrix obtained by replacing the value $-1$ with the weight $-w_{\none,\ntwo}$ on the edge $(\none,\ntwo)$ and the degree $d(\none)$ with the weighted degree.} 
as the \ac{gso}. 
The weights over the graph are drawn from a uniform distribution $U([0,1])$, and the rate is set to $r=1$.
The values assigned to the nonzero elements in the sparse graph signal, $\signal$, are drawn from the uniform distribution $U([-1,-0.5]\cup[0.5,1])$. 
The filtered signal, $\filter\xvec$, is normalized to obtain $\norm{\filter\signal}^2=\text{SNR}(\card{\nodes}\sigma_n^2)$, where SNR denotes the signal-to-noise ratio. The noise covariance matrix is set to $\Rmat=0.01^2\Imat$, and the SNR is set to $50$ unless defined otherwise.


\subsubsection{Methods}
The \ac{gbgic} and \ac{gmgic} methods were compared to several other methods, including: 
1) \ac{gic}, where an exhaustive search is performed to solve \eqref{eq; gic};
2) Lasso \cite{tibshirani1996regression}, where the $s$ indices of the solution with the highest absolute values are set as the estimated support; and
3) \ac{omp} \cite{elad2010sparse}. 
For each method mentioned above, we apply the \ac{gfoc} support recovery correction method presented in Algorithm \ref{alg; gfoc}. 
The corrected versions of these methods are denoted as follows:
$\overline{\ac{gbgic}}^{c}$, 
$\overline{\ac{gmgic}}^{c}$,
$\overline{\ac{gic}}^{c}$, $\overline{\text{lasso}}^{c}$, and $\overline{\ac{omp}}^{c}$.

\subsubsection{Tuning}
The penalty function used for the \ac{gbgic}, \ac{gmgic}, \ac{gic}, and \ac{gfoc} methods is the \ac{aic} penalty function, with $p(\card{\signalsupport})$ set to $2\card{\signalsupport}$.
For the \ac{gmgic} method, the pre-screening threshold $\rho$ is set to $\sigma_n$.
To estimate the support of the signal, the Lasso algorithm is applied multiple times with the tuning parameter $\lambda$ initialized to $20$ and then decreased until the estimated support $\hat{\signalsupport}$ satisfies either a) $\hat{\signalsupport}\ge \sparsityterm$, or b) $(\Imat-\proj{\hat{\signalsupport}})\measurements\le \card{\nodes}\sigma_n^2$ (for further information see Chapter 5.3.3 in \cite{elad2010sparse}).  
The \ac{omp} algorithm iterative procedure terminates when the estimated support satisfies either a) or b).

\subsection{Support Recovery Performance} \label{sec; sim; F-score}

The F-score classification metric, as described in \cite{sokolova}, is used to measure the performance of support recovery. It is defined as:
\begin{equation} 
FS(\signalsupport_t,\hat{\signalsupport})=\frac{2t_p}{2t_p+f_n+f_p},
\end{equation}
where $t_p$ represents the number of true-positives, $f_p$ represents the number of false-positives, and $f_n$ represents the number of false-negatives. These values are calculated based on the intersection between the true support, $\signalsupport_t$, and the estimated support, $\hat{\signalsupport}$. The F-score value ranges between 0 and 1, where a value of 1 indicates perfect support estimation.
\color{red} $1,000$ \color{black} Monte Carlo simulations were conducted.

\subsubsection{Framework 1 - $2$D-grid graph with $100$ vertices} \label{sec; sim; grid}
The support recovery methods performance, \ac{wrt} support estimation accuracy and run time, is examined 
for the two cases illustrated in Fig. \ref{fig; 2D} in which two different supports are selected for the sparse graph signal.
\begin{figure}[h!]
\centering 
 \includegraphics[trim={2cm 1.5cm 1.5cm 1cm},clip,width=6cm]{a_figures/2Dgraph.eps}
\caption{$2$D-graph with $\abs{\nodes}=100$ with the following cases: 1) $\signalsupport_{t}=\{1,10,91,100\}$ (red); and  2) $\signalsupport_{t}=\{45,46,55,56\}$ (blue). }
\label{fig; 2D}
\end{figure}
\begin{figure}[!b]
\centering
\begin{subfigure}[b]{0.5\textwidth}
\centering
  \includegraphics[width=5.5cm]{a_figures/conf1.eps}
 \caption{$\signalsupport_{t}=\{1,10,91,100\}$}
\end{subfigure}
\begin{subfigure}[b]{0.5\textwidth}
\centering
  \includegraphics[width=5.5cm]{a_figures/conf2.eps}
 \caption{ $\signalsupport_{t}=\{45,46,55,56\}$}
\end{subfigure}
\caption{$2$D graph: the F-score of the different methods are compared versus the graph filter degree, $\filterdeg$, for the two cases illustrated in Fig. $2D$.  } 
\label{fig; 2D-grid F-score verse degree}
\end{figure}  

Figure \ref{fig; 2D-grid F-score verse degree} shows the F-score for the two cases presented in Fig. \ref{fig; 2D}. In Fig. \ref{fig; 2D-grid F-score verse degree}.a, where $\signalsupport_{t}=\{1,10,91,100\}$, the F-scores of the graph-based methods, including \ac{gic}, \ac{gbgic}, \ac{gmgic}, and the \ac{omp} method, are almost equivalent. The F-score for these methods moderately decreases with the increase of the filter degree. On the other hand, the F-score of the Lasso method is lower by around $0.1$ when the graph filter is $1$ and decreases rapidly as the filter degree increases. In Fig. \ref{fig; 2D-grid F-score verse degree}.b, where $\signalsupport_{t}=\{45,46,55,56\}$, the \ac{gmgic} shows the closest F-score results to the optimal \ac{gic} method. The Lasso method obtains equivalent results to the \ac{gmgic} for the first and second degree but provides poor results for graph filter degrees higher than $2$. The \ac{gbgic} F-score comes close behind the \ac{gmgic} F-score, and they meet when the filter degree is $5$. In this case, the \ac{omp} method obtains low F-scores when the degree is higher than $1$.

As shown in Figure \ref{fig; 2D-grid F-score verse degree}, the \ac{gfoc} correction method has the potential to improve the support recovery results. 
In Fig. \ref{fig; 2D-grid F-score verse degree}.a, we can see that the Lasso method's results are significantly improved for all filter degrees when the \ac{gfoc} correction step is applied. The most significant improvement is seen when the filter degree is $3$, where the F-score increases from $0.6$ to $0.75$. However, for the other methods that already closely achieve the optimal benchmark set by the \ac{gic} method, applying the \ac{gfoc} correction does not improve the results. In Fig. \ref{fig; 2D-grid F-score verse degree}.b, the most significant improvement is observed for the \ac{omp} method. Additionally, the \ac{gbgic} method shows a significant improvement in graph degrees lower than $4$, where the corrected version, $\overline{\text{\ac{gbgic}}}^c$, obtains F-scores close to the \ac{gmgic} and \ac{gic} methods.


In Figure \ref{fig; 2D-grid SNR}, we also consider the case where $\{45,46,55,56\}$. 
However, this figure presents the F-score as a function of the SNR rate while the filter degree is set to $\filterdeg=4$. 
As shown in Figure \ref{fig; 2D-grid SNR}.a, the F-score of all methods improves as the SNR increases. 
The best performance is achieved by the proposed \ac{gmgic} and \ac{gbgic} methods, which are only slightly less effective than the optimal \ac{gic} method. Additionally, we observe that the \ac{gfoc} correction method is most effective when applied to the \ac{omp} method. 

\begin{figure}[h!]
\centering
\includegraphics[width=5.5cm]{a_figures/conf3.eps}
\caption{$2$D graph: the F-scores of the support recovery methods are compared versus the SNR rate for $\signalsupport_t=\{45,46,55,56\}$ and $\filterdeg=4$.}
\label{fig; 2D-grid SNR}
\end{figure}  

\subsection{Framework 2: Erd\H{o}s R\'eyni Graph with $70$ vertices} \label{sec; sim; erdus}
The performance of the different methods is examined over the realization (illustrated in Fig. \ref{fig; erdos}) obtained by drawing an Erd\H{o}s-R\'enyi graph of $70$ vertices 
with the probability of $0.12$ that two vertices are connected.
\begin{figure}[h!]
\centering 
 \includegraphics[trim={2.5cm 2cm 2cm 1cm},clip,width=5cm]{a_figures/ErdusGraph.eps}
\caption{Realization of an Erd\H{o}s-R\'enyi of $70$ vertices with probability of $0.12$ for two vertices to be connected.}
\label{fig; erdos}
\end{figure} 
The signal support has been selected randomly using the following two rules:
\begin{enumerate}[label=\textbf{Case.\arabic*}, leftmargin=1cm,topsep=2.5pt]
    \item \label{erdos; 1} \textbf{A group of four adjacent vertices:} A single vertex is randomly selected from the graph's vertex set. Then, three of the vertex's neighbors are randomly chosen.
    \item \label{erdos; 2} \textbf{Two groups of two adjacent vertices:} Two vertices are selected at random. Then, for each vertex, one of its neighbors is randomly chosen. This process is repeated until four different vertices are selected.
\end{enumerate}

In Figure \ref{fig; erdos performance}, we show the F-score obtained from the support recovery methods evaluated over the Erdős-Rényi graph realization depicted in Figure \ref{fig; erdos} as a function of the graph filter degree. 
It is evident from the results that the \ac{gmgic} method performs the best and is the closest to the optimal \ac{gic} method. The \ac{gbgic} method overall provides results closest to the \ac{gmgic}, except for lower degrees. Moreover, its corrected version, $\overline{\text{\ac{gbgic}}}^c$, produces even closer results to the \ac{gmgic} and \ac{gic} methods for all degrees. 
The Lasso method produces comparable results for lower degrees up to $2$. However, its F-scores decrease significantly for degrees higher than $2$. 
The \ac{omp} method provides comparative F-scores only for the first degree. However, its corrected version, $\overline{\text{\ac{omp}}}^c$, produces comparative F-scores for degrees lower than $4$.



\begin{figure}[h!]
\centering
\includegraphics[width=5.5cm]{a_figures/Reyni_united.eps}
\caption{Erd\H{o}s-R\'enyi Graph: the F-score of the different sparse support recovery methods with $\signalsupport$ chosen half of the time by \ref{erdos; 1} and half of the time by \ref{erdos; 2}.  } 
\label{fig; erdos performance}
\end{figure}  



\subsection{Complexity} \label{sec; sim; run}
The complexity of a method is measured by the run-time required to execute the method's algorithm. For our simulations, we used two Intel(R) Xeon(R) CPU E5-2660 v4 @ 2.00 GHz processors.

In Fig. \ref{fig; 2D-grid run time verse degree}, we can see the run-time required for different support recovery methods as a function of the graph filter degree, 
where $\signalsupport_t$ is chosen half of the time by $\signalsupport_t=\{1,10,91,100\}$ and half of the time by $\signalsupport_t=\{45,46,55,56\}$.
We observed that the run-time for the \ac{gmgic} and \ac{gbgic} methods increased as the filter degree increased. 
Additionally, for all degrees, the run-time required for \ac{gmgic} and \ac{gbgic} was higher than that required for the \ac{omp} and Lasso methods. However, it was still lower than the optimal \ac{gic} method's run-time. 
It can also be observed that the \ac{gbgic} required significantly less run-time compared to \ac{gmgic}. Furthermore, the addition of the \ac{gfoc} correction algorithm's run-time was very low and could be ignored.

\begin{figure}[h!]
\centering
  \includegraphics[width=5.5cm]{a_figures/Run_verse_Deg.eps}
\caption{$2$D graph: the run-time of the different methods are compared versus the graph filter degree with with $\signalsupport_t$ is chosen half of the time by $\signalsupport_t=\{1,10,91,100\}$ and half of the time by $\signalsupport_t=\{45,46,55,56\}$.}
\label{fig; 2D-grid run time verse degree}
\end{figure}

Figure \ref{fig; run time verse SNR} shows the run-time required for the different support recovery methods as a function of the SNR rate, with support and graph filter degree values set to $\signalsupport=\{45,46,55,56\}$ and $\filterdeg=4$, respectively.
Our observations indicate that the run-time for both the \ac{gmgic} and \ac{gbgic} methods increases as the SNR rate increases. 
In contrast, the run-time required for the \ac{gic} remains unchanged, and the run-time required for the \ac{omp} and Lasso methods slightly decreases. 
That said, both the \ac{gmgic} and \ac{gbgic} require significantly less run-time than the \ac{gic} method. 
Moreover, the \ac{gbgic} method works faster than the \ac{gmgic} method for all SNR rates.

\begin{figure}[h!]
\centering
  \includegraphics[width=5.5cm]{a_figures/conf3_Run.eps}
\caption{$2$D graph: the run-time of the different methods are compared versus the SNR for $\signalsupport=\{45,46,55,56\}$.}
\label{fig; run time verse SNR}
\end{figure}

Figure \ref{fig; run time verse graph size} presents the run-time required for the different support recovery methods as a function of graph size. In this case, the filter degree is set to $\filterdeg=4$, and the signal support is selected half the time as separated vertices and half the time as close vertices. For instance, the two cases are illustrated for the $2$D graph with $100$ vertices in Fig. \ref{fig; 2D}. Unlike the previous results in Fig. \ref{fig; 2D-grid run time verse degree} and \ref{fig; run time verse SNR}, the \ac{gbgic} and \ac{gmgic} methods' run-time does not change \ac{wrt} the graph size. The most significant change \ac{wrt} the graph size is observed for the \ac{gic} method, which is known to grow exponentially with the graph (model) size. As a result, the \ac{gbgic} and \ac{gmgic} methods are suitable for large networks.
It is worth noting that the F-score for all methods does not change \ac{wrt} the graph size.

\begin{figure}[h!]
\centering
  \includegraphics[width=5.5cm]{a_figures/Run_verse_graph_size.eps}
\caption{$2$D graph: the run-time of the different methods are compared versus the size of the graph.} 
\label{fig; run time verse graph size}
\end{figure}











\begin{comment}
   
\begin{figure*}[t!]
\centering
\begin{subfigure}[b]{0.31\textwidth}
\centering
  \includegraphics[width=5.5cm]{a_figures/conf3.eps}
 \caption*{a.1) F-score: $\signalsupport=\{1,10,91,100\}$}
\end{subfigure}
%\begin{subfigure}[b]{0.31\textwidth}
%\centering
% \includegraphics[width=5.5cm]{a_figures/conf2.eps}
% \caption*{b.1) F-score: $\signalsupport=\{2,10,55,56\}$}
%\end{subfigure} \hspace{\fill}
 \begin{subfigure}[b]{0.31\textwidth}
\centering
\includegraphics[width=5.5cm]{a_figures/conf1.eps}
\caption*{b.1) F-score: $\signalsupport=\{45,46,55,56\}$}
\label{fig; tau attacks}
\end{subfigure} \hspace{\fill}

\bigskip % more vertical separation
\begin{subfigure}[b]{0.31\textwidth}
\centering
  \includegraphics[width=5.5cm]{a_figures/conf3_Run.eps}
 \caption*{a.2) Run-time: $\signalsupport=\{1,10,91,100\}$}
\end{subfigure}
%\begin{subfigure}[b]{0.31\textwidth}
%\centering
 %\includegraphics[width=5.5cm]{a_figures/conf2_Run.eps}
 %\caption*{b.2) Run-time: $\signalsupport=\{2,10,55,56\}$}
%\end{subfigure} \hspace{\fill} 
\begin{subfigure}[b]{0.31\textwidth}
\centering
\includegraphics[width=5.5cm]{a_figures/conf1_Run.eps}
\caption*{b.2) Run-time: $\signalsupport=\{45,46,55,56\}$}
\label{fig; tau attacks}
\end{subfigure} \hspace{\fill}
\caption{ Analysis over the $2$D graph: the F-score and Run-time of the different methods are compared versus the graph filter degree, $\filter$, for different selections for the true signal support $\signalsupport_t$. \color{red} Fix notation and add the GIC method \color{black} } 
\label{fig; 2D-grid performance}
\end{figure*}    


%===========================================================%
%    Simulation variation for the Reyni graph framework     %
%===========================================================%

\begin{figure}[h!]
\centering
 
\begin{subfigure}[b]{0.5\textwidth}
\centering
\includegraphics[width=5.5cm]{a_figures/Reyni_conf2_Run.eps}
\caption{ Run-time: }
\label{fig; tau attacks}
\end{subfigure} \hspace{\fill}
\caption{ Erdus-Reyni Graph where of two groupd of two adjacent vertices are selected randomly as the signal support. } 
\label{fig; 2D-grid SNR}
\end{figure}  

\begin{figure}[h!]
\centering
 \begin{subfigure}[b]{0.5\textwidth}
\centering
\includegraphics[width=5.5cm]{a_figures/conf3_Run.eps}
\caption{2D-graph: $\signalsupport=\{1,10,91,100\}$}
\label{fig; tau attacks}
\end{subfigure} \hspace{\fill}
\begin{subfigure}[b]{0.5\textwidth}
\centering
\includegraphics[width=5.5cm]{a_figures/conf1_Run.eps}
\caption{2D-graph: $\signalsupport=\{45,46,55,56\}$ }
\label{fig; tau attacks}
\end{subfigure} \hspace{\fill}
\begin{subfigure}[b]{0.5\textwidth}
\centering
\includegraphics[width=5.5cm]{a_figures/Reyni_conf1_Run.eps}
\caption{ Reyni graph: group of $4$ neighbor nodes }
\label{fig; tau attacks}
\end{subfigure} \hspace{\fill}
\begin{subfigure}[b]{0.5\textwidth}
\centering
\includegraphics[width=5.5cm]{a_figures/Reyni_conf2_Run.eps}
\caption{ Reyni graph: two groupd of $2$ adjacant vertices}
\label{fig; tau attacks}
\end{subfigure} \hspace{\fill}

\caption{ Internal comparison of Run-Time figures } 
\label{fig; 2D-grid SNR}
\end{figure}  



\end{comment}



==> b_sections/h_conclusions.tex <==


\section{Conclusions}  \label{sec; conclusions}

In this work, we have introduce two new sparse recovery methods named \ac{gmgic} and \ac{gbgic}, 
which operate on graphical frameworks where a sparse input signal is evaluated from the outputs of a noisy graph filter. 
To improve the accuracy of the estimated support for the sparse input signal, 
we also presented a correction method called \ac{gfoc} that takes an estimated support obtained by any support recovery method as input and performs a low-complexity correction on it. All three methods are based on the well-known \ac{gic} criterion and take into account the structure of the graph and the double-sparsity imposed by both the graph and the graph signal.
We evaluated the performance of these methods, via Matlab simulations, and found that while \ac{gmgic} provides better support estimation performance than \ac{gbgic}, it comes at a higher computational cost. 
Nevertheless, both methods outperform the \ac{omp} and Lasso methods in terms of support estimation, with comparative run-time requirements. 
Additionally, the run-time required for both methods is significantly lower than the one required for the optimal GIC method that, in which an exhaustive search
is performed. 
Additionally, we witnessed that the \ac{gfoc} method improves the performance of the proposed and reference methods methods with a very low-complexity burden. 
The most significant improvement is recorded for the \ac{omp} and \ac{gbgic} methods. 
Specifically, by applying the \ac{gfoc} correction on the \ac{gbgic}, we obtained support estimation results comparable to the \ac{gic} benchmark, with comparative run-time to the \ac{omp} and Lasso methods.



==> d_candidates/theoretic_bounds.tex <==
%======================================================================================
%======================================================================================
%                                 Theoretic bounds 
%======================================================================================
%======================================================================================

%--------------Idea----------
% We would like to understanbd if we can provide theoretical bounds for the problem


\section{Bounds and Bounds}

\begin{defin}
    The mutual coherence of the $m\times n$ matrix $\Amat$ with the column set $\{\avec_i\}_{i=1}^n$ is given by 
    \be \label{eq; mutual coherence}
    \mu_{\Amat}=\underset{i\ne j}{max}~\frac{\lvert \avec_i^T\avec_j\rvert}{\|\avec_i\|\|\avec_j\|}.
    \ee
\end{defin}


\subsection{General}

\begin{hip} \label{hip; Laplacian coherence}
   The mutual coherence of the graph filter is higher with the increase in the filter degree, $\filterdeg$, \
   and for higher selection of the filter coeficient rate $\rate$. 
\end{hip}


\begin{comment}

\begin{thm}
   If $\mutualnot{\laplacian}=0$ and $\edge{\none}{\ntwo}\in\edges $ then
    $$
    \mutual{\submatcol{\filter}{\none}}{\submatcol{\filter}{\ntwo}} =  2\sum_{\iterone=2}^{\filterdeg} \rate^{\iterone}
    $$
\end{thm}
\begin{thm}
   If $\mutualnot{\laplacian}=0$ and $\edge{\none}{\ntwo}\notin\edges $ then
    $$
    \mutual{\submatcol{\filter}{\none}}{\submatcol{\filter}{\ntwo}}  < 2\sum_{\iterone=2}^{\filterdeg} \rate^{\iterone}
    $$
\end{thm}
\begin{cor}
    If $\mutualnot{\laplacian}=0$ then $\mutualnot{\filter}= 2\sum_{\iterone=2}^{\filterdeg} \rate^{\iterone}$. 
\end{cor}


\begin{proof}
    \color{red} we need to validate this. We also need to prove this.   \color{black}
\end{proof}
Special case: if $\rate=1$ then $\mutualnot{\filter}= 2\Psi$. \\
\color{blue}

What we are showing here is that if the filter degree is higher than one. The mutual coherence increases. 
In addition, we are trying to show the rate of increasment. 
This is the reason that the standard sparse approximation techniques performance deteriorates when the filter degree increases. 
This is also the reason the decay rate coefficient has a very important role. 
\color{black}
\end{comment}

\subsection{unweighted}
We consider the unweighted graph Laplacian matrix $\Lmat$ given by 
\be
L_{i,j}=\begin{cases} 
-1 & (i,j)\in\mathcal{E} \\
\lvert \mathcal{N}_1(i)\rvert & i=j \\
0 & \text{else}.
\end{cases}
\ee
We denote the columns of the Laplacian matrix by $\{\lvec_i\}$%_{i\in\mathcal{V}}$
For any $i,j\in\mathcal{V}$ we obtain
\be \label{eq; cool}
\lvec_i^T\lvec_j=\begin{cases}
\lvert\mathcal{N}_1(i)\rvert+\lvert \mathcal{N}_1(i)\rvert^2 & i=j \\
 -\lvert \mathcal{N}_1(i)\rvert-\lvert \mathcal{N}_1(j)\rvert & d(i,j)=1 \\
 +\lvert \mathcal{N}_1(i)\cap \mathcal{N}_1(j)\rvert   \\
\lvert \mathcal{N}_1(i)\cap \mathcal{N}_1(j)\rvert    & d(i,j)=2 \\
0 & d(i,j)>2    
\end{cases}
\ee
This is cool. Well we can bound \eqref{eq; cool} by 
\be \label{eq; cool}
\lvert\lvec_i^T\lvec_j\rvert\le\begin{cases}
\lvert\mathcal{N}_1(i)\rvert+\lvert \mathcal{N}_1(i)\rvert^2 & i=j \\
 \lvert \mathcal{N}_1(i)\rvert+\lvert \mathcal{N}_1(j)\rvert & d(i,j)=1 \\  
\min(\lvert \mathcal{N}_1(i)\rvert, \lvert\mathcal{N}_1(j)\rvert)    & d(i,j)=2 \\
0 & d(i,j)>2    
\end{cases}
\ee

\subsubsection{$d$-regular graphs}
Let $\lvert \mathcal{N}_1(i)\rvert=d, ~\forall i$. 
Then
\be
\mu_{\Lmat}=\frac{2d}{d(1+d)} =\frac{2}{1+d}. 
\ee
\subsection{Weighted}



\begin{defin}
 Let $\tilde{\Lmat}$ be the result of applying an $\ell_2$ normalization for the columns in $\Lmat$, 
 where $\Lmat$ is the graph Laplacian matrix of the graph $\mathcal{G}(\Vcal, \mathcal{E})$.
\end{defin}

%Now let $\tilde{\mathcal{G}}=(\Vcal,\mathcal{E})$ with the weights $\{\tilde{\omega}_e\}_{e\in\tilde{\mathcal{E}}}$ be the graph derived from $\tilde{\Smat}$ and denote
We denote the following notations
\be
\tilde{\omega}^e_{m}=\underset{i\ne j }{\max} -\tilde{L}_{i,j}
\ee

and 
\be
\tilde{\omega}^v_{m}=\underset{i}{\max} ~\tilde{L}_{i,i}. 
\ee

It can be easily verified that $\tilde{\omega}^e_{m}\le \tilde{\omega}^v_{m}$.

\begin{thm}
The mutual coherence of $\Lmat$ is bounded by 
\be
\mu^{\Smat}\le d_m\tilde{\omega}^e_{m}\tilde{\omega}^v_{m}
\ee
where $d_m$ is the maximal degree in $\mathcal{G}$.  \color{red} recheck maybe $d_m$ can be replaced by $2$. 
\end{thm}
\begin{proof}
    We consider $3$ cases: 1) $d(i,j)>2$; 2) $d(i,j)=2$; and $d(i,j)=1$. 
    For case $1$, $d(i,j)>2$, by substituting $\Psi=1$ in \eqref{eq; F prop 2} we obtain $\avec_i^T\avec_j=0$. 
    For case $2$, $d(i,j)=2$ we obtain that 
    \be
    \begin{aligned}
     - \frac{\avec_i^T\avec_j}{\|\avec_i\|\|\avec_j\|}&=\sum_{k:~(i,k),(j,k)\in\mathcal{E}} \frac{\omega_{i,k}}{\|\avec_i\|}\frac{\omega_{j,k} }
    {\|\avec_j\|}\\
      &\le d_m \underset{k}{\max} ~\frac{\omega_{i,k}}{\|\avec_i\|}\frac{\omega_{j,k} }
    {\|\avec_j\|} 
    \end{aligned}
    \ee
    This conveys that 
    \be
\mu_{\Lmat}\le  d_m\tilde{\omega}^e_{m}\tilde{\omega}^e_{m}\le d_m\tilde{\omega}^e_{m}\tilde{\omega}^v_{m}.
    \ee
    For case $3$, $d(i,j)=1$ we obtain that 
    \be
    \begin{aligned}
      \frac{ \avec_i^T\avec_j}{\|\avec_i\|\|\avec_j\|}&= \frac{\omega_{i,i}}{\|\avec_i\|}\frac{\omega_{j,i} }
    {\|\avec_j\|}  + \frac{\omega_{i,j}}{\|\avec_i\|}\frac{\omega_{j,j} }
    {\|\avec_j\|} \\
    &- \sum_{k:~(i,k),(j,k)\in\mathcal{E}} \frac{\omega_{i,k}}{\|\avec_i\|}\frac{\omega_{j,k} }
    {\|\avec_j\|}\\
    \end{aligned}
    \ee
\end{proof}
\color{red} split to two cases. positive and negative and bound each one. 
go over (11) again. maybe we can do something smarter there (more tight) 
\color{black}




==> e_observer/contemplate.tex <==
%======================================================================================
%======================================================================================
%                                 Contemplate 
%======================================================================================
%======================================================================================

%-----Idea-----
%This page includes the different things one should contemplate on. 

\section{Contemplate}

\subsection{Visualizations}
\begin{itemize}
    \item It could be interested to see a graph with the order of magnitude over the different projections. 
    \color{red} We can do this with colormap or something. \color{black}
    \item It could be cool to do a numerical investigation for the mutual coherence in different settings for the graph filter matrix and the graph Laplacian matrix. 
\end{itemize}

\subsection{Variations}

\begin{itemize}
\item Basically, the only thing which is not really inline is the selection of the lower bound in \eqref{eq_inequality single}. 
We can only change $(s-\lvert\Omega_1\rvert)\|\Pmat_{v_{k+1}} \yvec\|^2$ without changing the methodology.
We still need to ensure that this component is zero ($0$) when $\lvert \Omega_1 \rvert= 0$. 
However, I think it is fair to play a bit with this value and make it a bit bigger. 
\item Should we add a tuning parameter to the proposed method in a similar manner to the GIC and the GM-GIC methods? 
In other words, should we build the problem as a GIC problem instead of a sparse recovery problem? 
\end{itemize}


==> e_observer/instructions.tex <==

%======================================================================================
%======================================================================================
%                                 Instructions 
%======================================================================================
%======================================================================================

%-----Idea-----
%This page should include different instruction from collaborators or different things we want to commit in the manuscript


\color{blue}

\section{tirza}
Set the problem formulation like the conference paper. 
\section{changes}
\begin{itemize}
    \item Describe the changes in simulation. 
    \item e.g. the GM-GIC does not need historic data anymore. 
\end{itemize}



\color{black}

==> g_bios/Bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in, height=1.25in, trim=40pt 30pt 0pt 30pt, clip, keepaspectratio]{g_bios/Portraits/Gal_Morgenstern.png}}] {Gal Morgenstern}
is a Ph.D. research student in the School of Electrical and Computer Engineering at Ben-Gurion University of the Negev, Beer-Sheva, Israel. He received his B.Sc. (cum laude) and M.Sc. degrees in Electrical and Computer Engineering from Ben-Gurion University in 2019 and 2020, respectively. In 2019, he was awarded the Israeli Ministry of Science and Technology’s Zabutinsky scholarship, as well as the Kreitman Negev scholarship for his Ph.D. studies. In 2021, he was an exchange researcher at the Wireless \& Mobile Networking Lab (WiMNet) at Columbia University as part of the UN-funded Next Generation Internet (NGI) Explorers Program. His primary research interests include statistical signal processing and graph signal processing, with applications in power system cybersecurity.
\end{IEEEbiography}

\vspace{0.3cm}
\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1 in,height=1.25 in,clip,keepaspectratio]{g_bios/Portraits/Tirza_Routtenberg.png}}] {Tirza Routtenberg} 
 (Senior Member, IEEE) is an Associate Professor in the School of Electrical and Computer Engineering at Ben-Gurion University of the Negev, Israel. She received the B.Sc. degree from the Technion Israel Institute of Technology, Haifa, Israel, in 2005, and the M.Sc. and Ph.D. degrees in electrical and computer engineering in 2007 and 2012, respectively, from Ben-Gurion University, Israel. She was a Postdoctoral Fellow with the School of Electrical and Computer Engineering, Cornell University, in 2012-2014. Since October 2014, she has been a faculty member at the School of Electrical and Computer Engineering at Ben-Gurion University. In 2022–2023, she was a William R. Kenan, Jr. Visiting Professor for Distinguished Teaching at Princeton University. Her research interests include signal processing in smart grids, statistical signal processing, estimation and detection theory, and signal processing on graphs. She was an Associate Editor of IEEE Transactions on Signal and Information Processing Over Networks (2019 – 2023), Associate Editor of IEEE Signal Processing Letters (since 2021), and Subject Editor of Signal Processing ELSEVIER (since 2024), as well as a member of the IEEE Signal Processing Theory and Methods Technical Committee. She was a recipient of the Best Student Paper Award at the International Conference on Acoustics, Speech and Signal Processing (ICASSP) 2011,  IEEE International Workshop on Computational Advances in Multi-Sensor Adaptive Processing (CAMSAP) 2013 (coauthor),  ICASSP 2017 (coauthor), and IEEE Workshop on Statistical Signal Processing (SSP) 2018 (coauthor). She was awarded the Negev scholarship in 2008, the Lev-Zion scholarship in 2010, the Marc Rich Foundation Prize in 2011, and the Toronto Prize for Excellence in Research in 2021.
\end{IEEEbiography}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
